Robustly Learning Mixtures of $k$ Arbitrary Gaussians

We give a polynomial-time algorithm for the problem of robustly estimating a mixture of $k$ arbitrary Gaussians in $\mathbb{R}^d$, for any fixed $k$, in the presence of a constant fraction of arbitrary corruptions. This resolves the main open problem in several previous works on algorithmic robust statistics, which addressed the special cases of robustly estimating (a) a single Gaussian, (b) a mixture of TV-distance separated Gaussians, and (c) a uniform mixture of two Gaussians. Our main tools are an efficient \emph{partial clustering} algorithm that relies on the sum-of-squares method, and a novel \emph{tensor decomposition} algorithm that allows errors in both Frobenius norm and low-rank terms.

==> intro-old-conflicted.tex <==
%!TEX root = main.tex


\section{Introduction} \label{sec:intro}

\subsection{Background and Motivation} \label{ssec:background}

Given a collection of observations and a class of models, 
the objective of a typical learning algorithm is to find the model in the class that best fits the data.
The classical assumption is that the input data are i.i.d. samples generated by a statistical model 
in the given class. This is a simplifying assumption that is, at best, only approximately valid, as 
real datasets are typically exposed to some source of systematic noise. 
Robust statistics~\cite{HampelEtalBook86, Huber09} challenges this assumption by focusing
on the design of {\em outlier-robust}  estimators  --- algorithms 
that can tolerate a {\em constant fraction} of corrupted datapoints, independent of the dimension. 
Despite significant effort over several decades starting with important early works of Tukey and Huber in the 60s, 
even for the most basic high-dimensional estimation tasks,
all known computationally efficient estimators were until fairly recently highly sensitive to outliers.

This state of affairs changed with two independent works from the TCS community~\cite{DKKLMS16, LaiRV16},
which gave the first computationally efficient and outlier-robust learning algorithms for a range of ``simple''
high-dimensional probabilistic models. In particular, these works developed efficient robust estimators
for a single high-dimensional Gaussian distribution with unknown mean and covariance.
Since these initial algorithmic works~\cite{DKKLMS16, LaiRV16}, 
we have witnessed substantial research progress on algorithmic aspects of 
robust high-dimensional estimation by several communities of researchers, including TCS, machine learning,
and mathematical statistics. See Section~\ref{ssec:related} for an overview of the prior work most relevant
to the results of this paper. The reader is referred to~\cite{DK20-survey} for a  recent survey on the topic. 

One of the main original motivations for the development of algorithmic robust statistics within the TCS community 
was the problem of learning high-dimensional Gaussian mixture models.
A {\em Gaussian mixture model (GMM)} is a convex combination of Gaussian distributions, i.e.,
a distribution on $\R^d$ of the form $\calM  = \sum_{i=1}^k w_i \mathcal{N}(\mu_i, \Sigma_i)$, where
the weights $w_i$, mean vectors $\mu_i$, and covariance matrices $\Sigma_i$ are unknown.
GMMs are {\em the} most extensively studied latent variable model in the statistics and machine learning literatures, 
starting with the pioneering work of Karl Pearson in 1894~\cite{Pearson:94}, 
which introduced the method of moments in this context.

In the absence of outliers, a long line of work initiated by Dasgupta~\cite{Dasgupta:99, AroraKannan:01, VempalaWang:02, AchlioptasMcSherry:05, KSV08, BV:08} gave efficient clustering algorithms for GMMs under various separation assumptions. 
Subsequently, efficient learning algorithms were obtained~\cite{KMV:10, MoitraValiant:10, BelkinSinha:10, HardtP15} 
under minimal information-theoretic conditions. Specifically, Moitra and Valiant~\cite{MoitraValiant:10} and Belkin and Sinha~\cite{BelkinSinha:10} designed 
the first polynomial-time learning algorithms for arbitrary Gaussian mixtures with any fixed number of components.
These works qualitatively characterized the complexity of this fundamental learning problem in the noiseless setting.
Alas, all aforementioned algorithms are very fragile in the presence of corrupted data.
Specifically, a {\em single} outlier can completely compromise
their performance. 

Developing efficient learning algorithms for high-dimensional GMMs in the more realistic {\em outlier-robust} setting
--- the focus of the current paper --- has turned out to be significantly more challenging. 
This was both one of the original motivations and the main open problem 
in the initial robust statistics works~\cite{DKKLMS16, LaiRV16}. 
We note that~\cite{DKKLMS16} developed a robust density estimation algorithm 
for mixtures of {\em spherical} Gaussians --- a very special case of our problem
where the covariance of each component is a multiple of the identity --- 
and highlighted a number of key technical obstacles that need to be overcome in order to handle the general case.
Since then, a number of works have made algorithmic progress on important special cases of the general problem.
These include faster robust clustering for the spherical case under minimal separation 
conditions~\cite{HopkinsL18, KothariSS18, DiakonikolasKS18-mixtures}, 
robust clustering for separated (and potentially non-spherical) Gaussian mixtures~\cite{BK20, DHKK20}, 
and robustly learning {\em uniform} mixtures of two arbitrary Gaussian components~\cite{Kane20}.

This progress notwithstanding, the algorithmic task of robustly learning a mixture of a constant number
(or even two) arbitrary Gaussians (with arbitrary weights) 
has remained a central open problem in this field, as highlighted recently~\cite{DVW19-vignette}.

This discussion motivates the following question, whose resolution is the main
result of this work:

\begin{question} \label{q:robust-gmm}
Is there a $\poly(d, 1/\eps)$-time robust GMM learning algorithm, in the presence of an $\eps$-fraction of outliers, 
that has a dimension-independent error guarantee, for an arbitrary mixture of any constant number of arbitrary Gaussians on $\R^d$?
\end{question}


\subsection{Our Results} \label{ssec:results}

To formally state our main result, we define
the model of robustness we study.
We focus on the following standard data corruption model 
that generalizes Huber's contamination model~\cite{Huber64}. 

\begin{definition}[Total Variation Contamination Model] \label{def:adv}
Given a parameter $0< \epsilon < 1/2$ and a class of distributions $\mathcal{F}$ on $\mathbb{R}^d$, 
the \emph{adversary} operates as follows: The algorithm specifies the number of samples $n$.
The adversary knows the true target distribution $X \in \mathcal{F}$ and selects a distribution $F$ such that
$\dtv(F, X) \leq \eps$. Then $n$ i.i.d. samples are drawn from $F$ and are given as input to the algorithm.
%We say that a set of samples is {\em $\epsilon$-corrupted} if it is generated by this process.
\end{definition}


Intuitively, the parameter $\epsilon$ in Definition~\ref{def:adv} 
quantifies the power of the adversary. The total variation contamination 
model is strictly stronger than Huber's contamination model. 
Recall that in Huber's model~\cite{Huber64}, the adversary generates 
samples from a mixture distribution $F$ of the form $F = (1-\epsilon) X + \epsilon N$, 
where $X$ is the unknown target distribution and $N$ is an adversarially chosen noise distribution. 
That is, in Huber's model the adversary is only allowed to add outliers.

\begin{remark}
The {\em strong contamination model}~\cite{DKKLMS16} is a strengthening of 
the total variation contamination, where an adversary can see 
the clean samples and then arbitrarily replace an $\eps$-fraction of these points 
to obtain an $\eps$-corrupted set of samples.
Our robust learning algorithm succeeds in this strong contamination model, with the additional 
requirement that we can obtain two sets of independent $\eps$-corrupted samples from the unknown mixture. 
%(The second set is needed to run a hypothesis testing routine after we obtain a small list of candidate hypotheses.)
\end{remark}



In the context of robustly learning GMMs, we want to design an efficient algorithm 
with the following performance: Given a sufficiently large set of 
samples from a distribution that is $\eps$-close in total variation distance to an unknown GMM $\calM$ on $\R^d$, 
the algorithm outputs a hypothesis GMM $\widehat{\calM}$ such that with high probability 
the total variation distance $\dtv(\widehat{\calM}, \calM)$ is small. Specifically, we want 
$\dtv(\widehat{\calM}, \calM)$ to be only a function of $\eps$ and independent 
of the underlying dimension $d$.

%\medskip

The main result of this paper is the following:

\begin{theorem}[Main Result]\label{thm:main-informal}
There is an algorithm with the following behavior:
Given $\eps>0$ and a multiset of $n = d^{O(k)} \poly(\log(1/\eps))$ samples from a distribution $F$ on $\R^d$ such that
$\dtv(F, \calM) \leq \eps$, for an unknown target $k$-GMM $\calM = \sum_{i=1}^k w_i \mathcal{N}(\mu_i, \Sigma_i)$, 
the algorithm runs in time $d^{O(k)} \poly_k(1/\eps)$ and outputs a $k$-GMM hypothesis 
$\widehat{\calM}  = \sum_{i=1}^k \widehat{w}_i \mathcal{N}(\widehat{\mu}_i, \widehat{\Sigma}_i)$ 
such that with high probability we have that 
$\dtv(\widehat{\calM}, \calM ) \leq g(\eps, k)$. Here $g: \R_+ \times \Z_+ \to \R_+$ is a function such that
$\lim_{\eps \rightarrow 0} g(\eps, k) = 0$.
\end{theorem}

Theorem~\ref{thm:main-informal} gives the first polynomial-time {\em robust proper learning} algorithm, 
with dimension-independent error guarantee, for arbitrary $k$-GMMs, for any fixed $k$. 
This is the first polynomial-time algorithm for this problem, even for $k=2$.
%The function $f$ in the exponent of the runtime is $f(k) = k^{O(k^2)}$. 
The function $g$ quantifying the final error guarantee is $g(\eps, k) = 1/(\log(1/\eps))^{C_k}$, 
for some function $C_k$ that goes to $0$ when $k$ increases. Importantly, for any fixed $k$, 
the final error guarantee only scales with $\eps$ and is independent of the dimension $d$. In Theorem~\ref{thm:robust-GMM-arbitrary-poly-eps}, we show that modifying a subroutine in our algorithm allows us improve this error to a fixed polynomial in $\epsilon$ which turns out to be almost optimal for any robust proper learning algorithm. 

It is worth pointing out that a $d^{\Omega(k)}$ lower bound in the running time is inherent for Statistical Query (SQ)
algorithms, even in the case when there are no outliers and the components 
of the mixture are pairwise separated in total variation distance~\cite{DKS17-sq}.

In an independent and concurrent work, Liu and Moitra~\cite{LM20} obtained a closely related result. Their algorithm makes stronger assumptions on the input mixture (lower bound on weights, singular values of the covariances and separation between mixture components) and obtains a formally stronger \emph{parameter estimation} guarantee. We discuss this in more detail in Section~\ref{ssec:related}. 

Our work is most closely related to the very recent paper by Kane~\cite{Kane20}, 
which gave a polynomial-time robust learning algorithm for the {\em uniform} $k=2$ case, 
i.e., the case of two {\em equal weight} components, and the polynomial time algorithms~\cite{BK20, DHKK20} for the problem under the (strong) assumption that the component Gaussians are pairwise well-separated in total variation distance. 

Our algorithm handles the case of arbitrary weights, and, most importantly, 
extends to any number of components $k$. 
We note that for the special case of uniform mixtures (or, more generally, mixtures whose weights are bounded below 
by a fixed function of $k$),  a much simpler application of our main tools suffices to resolve 
the problem (see Theorem~\ref{thm:robust-GMM-equiweigthed} for details). 
It is also worth noting that (for the case of uniform $2$-mixtures) 
the algorithm of Kane~\cite{Kane20} achieves a final error of $\poly(\eps)$, 
which is a quantitatively stronger error guarantee than that of Theorem~\ref{thm:main-informal}.

The works~\cite{BK20, DHKK20} give efficient 
clustering algorithms for any fixed number $k$ of components,  under the crucial assumption 
that the components have pairwise total variation distance close to $1$. 
In this case, one can hope (and, indeed, that is what the above works accomplish) 
to efficiently \emph{cluster} the input sample into $k$ groups, 
such that each group contains the samples generated from one of the Gaussians, 
up to some small misclassification error. In contrast, the challenge in the setting 
without separation assumptions is that it is information-theoretically impossible 
to cluster the samples. As we will explain in the proceeding
discussion, while we draw ideas from~\cite{BK20, DHKK20, Kane20}, 
a number of significant conceptual and technical challenges need to be overcome 
in the non-clusterable setting. 

In the noiseless case, the first polynomial-time learning algorithm for $k$-GMMs on $\R^d$ 
was given in~\cite{MoitraValiant:10, BelkinSinha:10}. 
In particular, the sample complexity and running time of the~\cite{MoitraValiant:10} algorithm is $(d/\eps)^{q(k)}$, 
for some function $q(k) = k^{\Omega(k)}$. As we explain in detail in the proceeding discussion, 
the \cite{MoitraValiant:10, BelkinSinha:10} algorithms are very sensitive to outliers 
and an entirely new approach is required to obtain an efficient  robust learning algorithm.

\paragraph{Improving Error to a Fixed Polynomial in $\epsilon$} 

The upshot of Theorem~\ref{thm:main-informal} is that it worke under information-theoretically least restricted assumptions. However, it only yields a inverse polylogarithmic error in $1/\epsilon$. It turns out that this can be traced entirely to a exhaustive search subroutine in the first component of that introduces a novel tensor decomposition subroutine. By a relatively straightforward upgrade that replaces this exhaustive search subroutine with a standard \emph{noiseless} GMM learning algorithm, we can actually obtain the nearly optimal $\poly(\epsilon)$ error. This is the content of the our second theorem below. 

\begin{theorem}[Robustly Learning $k$-Mixtures with $\poly(\epsilon)$-error, see Corollary \ref{thm:robust-GMM-arbitrary-poly-eps}] 
Given $0< \epsilon < 1/k^{k^{O(k^2)}}$ and a multiset $Y = \{ y_1, y_2, \ldots , y_n\}$ of $n$ i.i.d. 
samples from a distribution $F$ such that $\dtv(F, \calM) \leq \eps$,
%$\epsilon$-corrupted samples 
for an unknown $k$-mixture of Gaussians $\calM = \sum_{i \leq k} w_i\calN\Paren{\mu_i, \Sigma_i}$, 
where \new{$n \geq n_0=d^{O(k)}/\poly(\eps)$,} there exists an algorithm that runs 
\new{in time $d^{O(k)}\poly\left(k/\eps\right)$}
and with probability at least $0.99$ outputs a hypothesis $k$-mixture of Gaussians 
$\widehat{\calM} = \sum_{i \leq k} \hat{w}_i \calN\Paren{\hat{\mu_i}, \hat{\Sigma}_i}$ 
such that $d_{\textrm{TV}}\Paren{\calM, \widehat{\calM}} = \bigO{\eps^{c_k}}$, 
with $c_k=1/(100^k C^{(k+1)!}k!\mathrm{sf}(k+1))$, where $C>0$ is a universal constant 
and $\mathrm{sf}(k)=\Pi_{i \in[k]}(k-i)!$ is the super-factorial function.  
\end{theorem} 

Finally, we show that the \emph{same} algorithm as in Theorems~\ref{thm:main-informal} and \ref{thm:robust-GMM-arbitrary-poly-eps} actually implies that the recovered mixture of Gaussian is close in \emph{parameter} distance to the unknown mixture. 

Notice, of course, that uniquely recovering the parameters of the unknown mixture has to be clearly impossible if the components are not pairwise separated in an appropriate sense. Thus, parameter estimation results usually make a separation assumption on the mixture components. 

We adopt a more liberal stance and prove a stronger result that allows \emph{partial recovery} of parameters and in some sense, can be thought of as giving a guarantee of recovering whatever subset of parameters that can information theoretically be recovered. 

More specifically, in the theorem below, we prove that whenever the components of the input mixture can be clustered together into some groups so that all mixtures in a group are close (and thus, indistinguishable), there's a similar clustering of the output mixture such that all parameters (weight, mean and covariances) of each cluster are close within $\poly(\epsilon)$ in total variation distance. 

We stress that this is a purely information theoretic result -- the theorem below simply provides an additional stronger guarantee that the output of our main theorems (Theorem~\ref{thm:main-informal} and Theorem~\ref{thm:robust-GMM-arbitrary-poly-eps}).

\begin{theorem}[Parameter Recovery]
%There is an algorithm with the following behavior:
Given $\eps>0$ and a multiset of $n = d^{O(k)} \poly(1/\eps)$ samples from a distribution $F$ on $\R^d$ such that
$\dtv(F, \calM) \leq \eps$, for an unknown target $k$-GMM $\calM = \sum_{i=1}^k w_i \mathcal{N}(\mu_i, \Sigma_i)$, 
the algorithm runs in time $d^{O(k)} \poly_k(1/\eps)$ and outputs a $k'$-GMM hypothesis 
$\widehat{\calM}  = \sum_{i=1}^{k'} \widehat{w}_i \mathcal{N}(\widehat{\mu}_i, \widehat{\Sigma}_i)$ with $k'\le k$
such that with high probability we have that 
there exist a partition of $[k]$ into $k'+1$ sets $R_0,R_1,\dots,R_{k'}$ such that
\begin{enumerate}
\item 
Let $W_i=\sum_{j\in R_i}w_j$. 
Then for all $i\in[k']$,
\begin{align*}
|W_i-\hat w_i|&\le\poly(\epsilon)\\
\dtv(\mathcal{N}(\mu_j, \Sigma_j),\mathcal{N}(\widehat{\mu}_i, \widehat{\Sigma}_i))&\le\poly(\epsilon)\quad \forall j\in R_i
% \norm{\mu_j-\hat\mu_{\pi(i)}},\norm{\Sigma_j-\hat\Sigma_{\pi(i)}}_F&\le\poly(\epsilon)
\end{align*}
\item
The sum of weights of exceptional components in $R_0$ is at most $\poly(\epsilon)$.
\end{enumerate}
\end{theorem}

%\inote{Stuff below could be removed or moved to the appropriate section.}
%It is worth pointing out that the non-robust learning algorithm in~\cite{MoitraValiant:10} also solves the parameter estimation
%variant of the learning problem (as opposed to proper learning). In parameter estimation, it is assumed that the components
%are non-trivially separated in parameter distance, and the goal is to approximate the hidden parameters $w_i, \mu_i, \Sigma_i$ (up to a permutation) within small error. \new{Our algorithm can be used to obtain a list-decodable version of this problem, i.e., it outputs a small list of candidate hypotheses with the guarantee that one of them is close to the target mixture in parameter distance. While this guarantee does not immediately imply parameter estimation, we note that such a result would follow from our algorithm assuming a multi-dimensional robust identifiability result relating the parameter distance of two Gaussian mixtures and their total variation distance. \cite{MoitraValiant:10} proved such a structural result for the univariate case. While we do not prove a multi-dimensional analogue of the \cite{MoitraValiant:10} structural result in this paper, we note that such a result in {\em necessary} for parameter estimation to be information-theoretically possible with $\poly(d, 1/\eps)$ samples.}


%\snote{we could possibly add outline of challenges here, overall challenges, not just latest ones.}






==> lower-bound-eigenvalue-proof.tex <==
\begin{lemma}
Suppose are $N(\mu_1,\Sigma_1),N(\mu_2,\Sigma_2)$ are two Gaussians with $\norm{\mu_1-\mu_2}\le\delta$ and $\norm{\Sigma_1-\Sigma_2}_F\le\delta$. If eigenvalues of $\Sigma_1$ and $\Sigma_2$ are at least $\lambda<1$, then 
$$
\dtv(N(\mu_1,\Sigma_1),N(\mu_2,\Sigma_2))=O(\delta/\lambda).
$$
\end{lemma}

\begin{proof}
By Fact~\ref{GaussianTVFact}, we have 
$$
\dtv(N(\mu_1,\Sigma_1),N(\mu_2,\Sigma_2)) = O(((\mu_1-\mu_2)\cdot \Sigma_1^{-1} (\mu_1-\mu_2))^{1/2}+\|\Sigma_1^{-1/2}\Sigma_2 \Sigma_1^{-1/2}-I \|_F ).
$$
Then the first term is $\left((\mu_1-\mu_2)\cdot \Sigma_1^{-1} (\mu_1-\mu_2)\right)^{1/2}\le (\norm{\Sigma_1^{-1}}_2\norm{\mu_1-\mu_2}^2)^{1/2}\le\delta/\sqrt{\lambda}$.
The second term is 
\begin{align*}
\|\Sigma_1^{-1/2}\Sigma_2 \Sigma_1^{-1/2}-I \|^2_F
&=\norm{\Sigma_1^{-1/2}(\Sigma_1-\Sigma_2)\Sigma_1^{-1/2}}^2_F\\
&=\tr\left(\left(\Sigma_1^{-1/2}(\Sigma_1-\Sigma_2)\Sigma_1^{-1/2}\right)^2\right)\\
&\le\tr\left((\Sigma_1-\Sigma_2)^2\right)(1/\lambda)^2\\
&\le(\delta/\lambda)^2.
\end{align*}
Thus, 
$$
\dtv(N(\mu_1,\Sigma_1),N(\mu_2,\Sigma_2))=O(\delta/\sqrt{\lambda}+\delta/\lambda)=O(\delta/\lambda).
$$
\end{proof}


==> partial-clustering-copy.tex <==
%!TEX root = main.tex

\section{Robust Partial Cluster Recovery}
\label{sec:robust-partial-clustering} 
In this section, we give two robust \emph{partial clustering} algorithms. 
A partial clustering algorithm takes a set of points $X = \cup_{i \leq k}X_i$ 
with true clusters $X_1, X_2, \ldots, X_k$ and outputs a partition of the sample $X = X'_1 \cup X'_2$ such that $X'_1= \cup_{i \in S} X_i$ and 
$X'_2 = \cup_{i \not \in S} X_i$, 
for some subset $S \subseteq [k]$ of size $1 \leq |S| < k$. 
That is, a partial clustering algorithm partitions the sample into two non-empty parts 
so that each part is a sample from a ``sub-mixture''. This is a weaker guarantee than clustering 
that must find the original $X_i$'s and can be feasible to obtain even when the mixture as a whole 
is not clusterable. In our setting, we will get an approximate (that is, a small fraction of points are misclassified) partial clustering that works for $\epsilon$-corruptions $Y$ of any i.i.d. sample $X$ 
from a mixture of $k$ Gaussians, as long as there is a pair of components in the original mixture 
that have large total variation distance between them. 
%\Pnote{this discussion should appear in overview perhaps.}

A partial clustering algorithm such as above was one of the innovations in~\cite{BK20} 
that allowed for a polynomial-time algorithm for clustering all fully clusterable Gaussian mixtures. 
In particular,  their partial clustering subroutine was crucial in handling mixtures of Gaussians 
where some components have rank deficient covariances (i.e., $0$ variance in some directions). 

In this section, we  build on the ideas in~\cite{BK20} to derive two new partial clustering algorithms 
that work even when the original mixture is not fully clusterable. In order to state the guarantees of our algorithm, 
we first formulate a notion of parameter separation 
(same as the one employed in~\cite{BK20,DHKK20}) as the next definition.

\begin{definition}[$\Delta$-Parameter Separation] \label{def:separated-mixture-model}
We say that two Gaussian distributions $\cN(\mu_1,\Sigma_1)$ and $\cN(\mu_2,\Sigma_2)$ 
are $\Delta$-parameter separated if at least one of the following three conditions hold:
\begin{enumerate}
  \item \textbf{Mean-Separation:} $\exists v \in \R^d$ such that 
  $\langle \mu_1 - \mu_2, v \rangle^2 > \Delta^2 v^{\top} (\Sigma_1 + \Sigma_2) v$,
  \item \textbf{Spectral-Separation:} $\exists v \in \R^d$ such that $v^{\top} \Sigma_1 v > \Delta \, v^{\top}\Sigma_2v$,
  \item \textbf{Relative-Frobenius Separation:} $\Sigma_i$ and $\Sigma_j$ have the same range space and $\Norm{ \Sigma_1^{\dagger/2} (\Sigma_2 - \Sigma_1) \Sigma_1^{\dagger/2}}^2_F > \Delta^2 \Norm{\Sigma_1^{\dagger} \Sigma_2}_{\mathrm{op}}^2$.
\end{enumerate}
\end{definition}
As shown in ~\cite{DHKK20,BK20}, if a pair of Gaussians is $(1-\exp(-O(\Delta \log \Delta))$-separated in total variation distance, then, they are $\Delta$-parameter separated. 

%\Pnote{add def for pseudo-inverse to preliminaries}\Anote{this exists.}

Our first algorithm succeeds in robust partial clustering whenever there is a pair of component Gaussians that are 
$\Delta$-parameter separated. The running time of this algorithm grows exponentially 
in the reciprocal of the minimum weight in the mixture.  

\begin{theorem}[Robust Partial Clustering in TV Distance] \label{thm:partial-clustering-non-poly}
Let $0 \leq \epsilon < \alpha \leq 1$, and $\eta > 0$.  There is an algorithm with the following guarantees: 
Let $\{\mu_i,\Sigma_i\}_{i \leq k}$ be means and covariances of $k$ unknown Gaussians. 
Let $Y$ be an $\epsilon$-corruption of a sample $X$ of size $n\geq \paren{dk}^{Ct}/\epsilon$ for a large enough constant $C>0$, from $\calM = \sum_i w_i \cN(\mu_i,\Sigma_i)$ satisfying Condition~\ref{cond:convergence-of-moment-tensors} with parameters $t = (k/\eta)^{O(k)}$ and 
$\gamma \leq \epsilon d^{-8t}k^{-Ct}$, for a sufficiently large constant $C>0$.  
Suppose further that $w_i \geq \alpha > 2\epsilon$ for every $i$ and that 
there are $i, j$ such that $\cN(\mu_i,\Sigma_i)$ and $\cN(\mu_j,\Sigma_j)$ 
are $\Delta$-parameter separated for $\Delta = (k/\eta)^{O(k)}$. 

Then, the algorithm on input $Y$,
runs in time $n^{(k/\eta)^{O(k)}}$, and with probability at least $\alpha^{O(k \log \frac{k}{\eta \alpha})}$ 
over the draw of $X$ and the algorithm's random choices, 
the algorithm outputs a partition of $Y$ into $Y_1,Y_2$ satisfying: 
\begin{enumerate}
 \item \textbf{Partition respects clustering:} for each $i$, 
 $\max \{ \frac{k}{n}|Y_1 \cap X_i|, \frac{k}{n}|Y_2 \cap X_i|\} \geq 1-\eta- O(\eps/\alpha^4)$, and, 
 \item \textbf{Partition is non-trivial:} $\max_{i}\frac{k}{n} |X_i \cap Y_1|, \max_{i}\frac{k}{n} |X_i \cap Y_2| \geq 1-\eta-O(\eps/\alpha^4)$. 
\end{enumerate}
\end{theorem}

Our proof of the above theorem is based on a relatively straightforward extension of the ideas of~\cite{BK20} 
with the key upgrade that allows the input mixtures to have arbitrary mixing weights 
(at an exponential cost in the inverse of the minimum weight). The running time of the algorithm 
is prohibitively large (and not polynomial in the inverse of the mixing weights) 
when the one of the clusters has very small size. Unfortunately, it also appears that such a cost 
might be necessary in the setting of the above theorem. 

In order to get our main result that gives a fully polynomial algorithm (including in the inverse mixing weights), 
we will use a incomparable variant of the above partial clustering method that only handles 
a weaker notion of parameter separation, but runs in fixed polynomial time.

\begin{theorem}[Robust Partial Clustering in Relative Frobenius Distance] \label{thm:partial-clustering-poly}
Let $0 \leq \epsilon < \alpha/k \leq 1$ and $t \in \N$. There is an algorithm with the following guarantees: 
Let $\{\mu_i,\Sigma_i\}_{i \leq k}$ be means and covariances of $k$ unknown Gaussians. 
Let $Y$ be an $\epsilon$-corruption of a sample $X$ of size $n\geq \paren{dk}^{Ct}/\epsilon$ for a large enough constant $C>0$, from 
$\calM = \sum_i w_i \cN(\mu_i,\Sigma_i)$ that satisfies Condition~\ref{cond:convergence-of-moment-tensors} 
with parameters $2t$ and $\gamma \leq \epsilon d^{-8t}k^{-Ck}$, for a large enough constant $C >0$. 
Suppose further that $w_i \geq \alpha > 2 \epsilon$ for each $i \in [k]$, 
and that for some $t \in \N$, $\beta > 0$ there exist $i,j \leq k$ such that 
$\Norm{\Sigma^{\dagger/2}(\Sigma_i -\Sigma_j)\Sigma^{\dagger/2}}_F^2 = \Omega\left((k^2 t^4)/(\beta \alpha^4)^{2/t}\right)$, 
where $\Sigma$ is the covariance of the mixture $\calM$. 
Then, the algorithm runs in time $n^{O(t)}$, and with probability at least $\alpha^{O(k \log \frac{k}{\eta})}$ over the random choices of the algorithm, 
outputs a partition $Y = Y_1 \cup Y_2$ satisfying:   
\begin{enumerate}
 \item \textbf{Partition respects clustering:} for each $i$, $\max \{ \frac{1}{w_i n}|Y_1 \cap X_i|, \frac{1}{w_i n}|Y_2 \cap X_i|\} \geq 1- \beta - O(\epsilon/\alpha^4)$, and, 
 \item \textbf{Partition is non-trivial:} $\max_{i}\frac{1}{w_i n} |X_i \cap Y_1|, \max_{i}\frac{1}{w_i n} |X_i \cap Y_2| \geq 1- \beta - O(\epsilon/\alpha^4)$. 
\end{enumerate}
\end{theorem}

The starting point for the proof of the above theorem is the observation that the running time of our first algorithm above is exponential in the inverse mixing weight almost entirely because of dealing with spectral separation 
(which requires the use of ``certifiable anti-concentration'' that we define in the next subsection). 
We formulate a variant of relative Frobenius separation (that is directly useful to us) and prove that 
whenever the original mixture has a pair of components separated in this notion, 
we can in fact obtain a fully polynomial partial clustering algorithm building on the ideas in~\cite{BK20}. 


% Our partial clustering algorithm is based on the robust clustering algorithm introduced in~\cite{DHKK20,BK20} (we follow the treatment in ~\cite{BK20} here). The algorithm of~\cite{BK20} succeeds in clustering a mixture of any distributions that satisfy two analytic properties that we define in the next subsection. 




% The clustering algorithm of~\cite{BK20} work for mixtures of any distribution that satisfy two analytic notions that we next define. 




% Let $\sum_{i = 1}^n w_i \cN(\mu_i, \Sigma_i)$ be a $d$-dimensional mixture of Gaussians with $w_i \geq \alpha$ for every $i$. Let $\mu = \sum_i w_i \mu_i$ and $\Sigma = \sum_i w_i \Sigma_i + \sum_i w_i \bar{\mu}_i\bar{\mu}_i^{\top}$ for $\bar{\mu}_i = \mu_i - \mu$. 

% Let $X = \{x_1, x_2, \ldots, x_n\}$ be an i.i.d. sample of size $n$ drawn according to $\sum_{i = 1}^n w_i \cN(\mu_i, \Sigma_i)$ with true clusters $C_1, C_2, \ldots, C_k$. By a slight abuse of notation, we always think of $X$ as being generated by taking i.i.d. sample from $\cN(\mu_i,\Sigma_i)$ of size $w_i n$ for each $i$ and then taking the union of all such points. This allows us to conclude that $|X_i| = w_i n$ for each $i$. 

% Let $Y \subseteq \R^d$ of size $|Y| = n$ such that $|Y \cap X| \geq (1-\epsilon)n$. 



\subsection{Algorithm}

Our algorithm will solve SoS relaxations of a polynomial inequality system. 
The constraints here use the input $Y$ to encode finding a sample $X'$ 
(the intended setting being $X'=X$, the original uncorrupted sample) 
and a cluster $\hat{C}$ in $X'$ of size $= \alpha n$, indicated by $z_i$s 
(the intended setting is simply the indicator for any of the $k$ true clusters) 
satisfying properties of Gaussian distribution (certifiable hypercontractivity and anti-concentration). 


Covariance constraints introduce a matrix valued indeterminate intended to be the square root of $\Sigma$.
\begin{equation}
\text{Covariance Constraints: $\cA_1$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\Pi
      &=UU^{\top}\\
      % &
      % &\Theta \Pi = \Pi \Theta
      % &= I\\
      &
      &\Pi^2
      &=\Sigma\\
      % &
      % &\Theta^2\Sigma  = \Sigma \Theta^2
      % &=\Theta\Sigma\Theta =I\\
    \end{aligned}
  \right \}
\end{equation}
The intersection constraints force that $X'$ be $\epsilon$-close to $Y$ (and thus, $2\epsilon$-close to unknown sample $X$). 
\begin{equation}
\text{Intersection Constraints: $\cA_2$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &\forall i\in [n],
      & m_i^2
      & = m_i\\
      &&
      \textstyle\sum_{i\in[n]} m_i 
      &= (1-\epsilon) n\\
      &\forall i \in [n],
      &m_i (y_i-x'_i)
      &= 0
    \end{aligned}
  \right \}
\end{equation}
The subset constraints introduce $z$, which indicates the subset $\hat{C}$ intended to be the true clusters of $X'$.
\begin{equation}
\text{Subset Constraints: $\cA_3$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &\forall i\in [n].
      & z_i^2
      & = z_i\\
      &&
      \textstyle\sum_{i\in[n]} z_i 
      &= \alpha n\\
    \end{aligned}
  \right \}
\end{equation}

Parameter constraints create indeterminates to stand for the covariance $\Sigma$ and mean $\mu$ of $\hat{C}$ (indicated by $z$).
\begin{equation}
\text{Parameter Constraints: $\cA_4$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\frac{1}{\alpha n}\sum_{i = 1}^n z_i \Paren{x'_i-\mu}\Paren{x'_i-\mu}^{\top}
      &= \Sigma\\
      &
      &\frac{1}{\alpha n}\sum_{i = 1}^n z_i x'_i
      &= \mu\\
    \end{aligned}
  \right \}
\end{equation}

      % &
      % &\frac{1}{n}\sum_{i = 1}^n w_i x_ix_i^{\top}
      % &= \Sigma\\
      % &
      % &\frac{1}{n}\sum_{i = 1}^n w_i x_i
      % &= \mu\\



\text{Certifiable Hypercontractivity : $\cA_4$}=\\
\begin{equation}
 % \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
     &\forall j \leq 2s
     &\frac{1}{\alpha^2 n^2} \sum_{i,j \leq n} z_i z_j Q(x'_i-x'_j)^{2j}
     &\leq (Cj)^{2j}2^{2j}\Norm{\Pi Q \Pi}_F^{2j}\\
     &
     &\nnnew{\frac{1}{\alpha^2 n^2} \sum_{i,j \leq n} z_i z_j \Paren{Q(x'_i-x'_j)-\frac{1}{\alpha^2 n^2} \sum_{i,j \leq n} z_i z_j Q(x'_i-x'_j)}^{2}}
     &\nnnew{\leq 6\Norm{\Pi Q \Pi}_F^{2}}
    \end{aligned}
  \right \}
\end{equation}

In the constraint system for our first algorithm, we will use the following certifiable anti-concentration constraints on $\hat{C}$ for $\delta = \alpha^{-\poly(k)}$ and $\tau = \alpha/\poly(k)$ and $s(u) = 1/u^2$ for every $u$.
\begin{equation}
\text{Certifiable Anti-Concentration : $\cA_5$} =% \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      % &\forall i,j\in [n].
      % & w_i w_j \Paren{\norm{v}_2^{2t-2} \Iprod{\Paren{\frac{x_i-x_j}{\sqrt{2}}},v}^2 +\delta^2 p^2 (\Iprod{\Theta \Paren{\frac{x_i-x_j}{\sqrt{2}}},,v})}
      % &\geq w_i w_j \Paren{\delta^2 \norm{v}_2^{2t}}\\
      &
      &\frac{1}{\alpha^2 n^2}\sum_{i,j=  1}^n z_i z_j q_{\delta,\Sigma}^2\left(\Paren{x'_i-x'_j},v\right)
      &\leq 2^{s(\delta)} C\delta \Paren{v^{\top}\Sigma v}^{s(\delta)}\\
      &
      &\frac{1}{\alpha^2 n^2}\sum_{i,j=  1}^n z_i z_j q_{\tau,\Sigma}^2\left(\Paren{x'_i-x'_j},v\right)
      &\leq 2^{s(\tau)} C\tau \Paren{v^{\top}\Sigma v}^{s(\eta)}\\
     \end{aligned}
    \right\}
 \end{equation}

 In the constraint system for our second algorithm, we will not use $\cA_5$.
 %and instead force the following constraints on the parameters of the mixture:
% \begin{equation}
% \text{Mixture Parameters : $\cA_6$} =% \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       % &\forall i,j\in [n].
%       % & w_i w_j \Paren{\norm{v}_2^{2t-2} \Iprod{\Paren{\frac{x_i-x_j}{\sqrt{2}}},v}^2 +\delta^2 p^2 (\Iprod{\Theta \Paren{\frac{x_i-x_j}{\sqrt{2}}},,v})}
%       % &\geq w_i w_j \Paren{\delta^2 \norm{v}_2^{2t}}\\
%       &
%       &\frac{1}{n^2}\sum_{i,j=  1}^n  (x_i'- x_j')(x_i'-x_j')^{\top}
%       &= 4 \Sigma \\
%       &
%       &0.99 I \preceq \Sigma 
%       &\preceq 1.01I\\
%      \end{aligned}
%     \right\}
%  \end{equation}



Our algorithms for proving Theorems~\ref{thm:partial-clustering-poly} and~\ref{thm:partial-clustering-non-poly} will both use the following algorithm that differs only in the degree of the pseudo-distribution computed and the constraint system that the pseudo-distribution satisfies. 

\begin{mdframed}
  \begin{algorithm}[Partial Clustering]
    \label{algo:robust-partial-clustering}\mbox{}
    \begin{description}
    \item[Given:]
        A sample $Y$ of size $n$. An outlier parameter $\epsilon > 0$ and an accuracy parameter $\eta > 0$. 
    \item[Output:]
      A partition of $Y$ into partial clustering $Y_1 \cup Y_2$.
    \item[Operation:]\mbox{}
    \begin{enumerate}
    	%\item \textbf{Base Case:} If $|Y'| = n/k$, accept if Algorithm~\ref{algo:verification-subroutine} applies to $Y'$ with outlier parameter $\tau$ accepts. Otherwise output fail.
   		\item \textbf{SDP Solving:} Find a pseudo-distribution $\tzeta$ satisfying $\cup_{i =1}^5 \cA_i$ ($\cup_{i = 1}^4 \cA_i$ for Theorem~\ref{thm:partial-clustering-poly}) such that $\pE_{\tzeta}z_i \leq \alpha$ for every $i$. If no such pseudo-distribution exists, output fail.
      	\item \textbf{Rounding:} Let $M = \pE_{z \sim \tzeta} [zz^{\top}]$. 
       		\begin{enumerate} 
        		 \item Choose $\ell = O(\frac{1}{\alpha} \log (k/\eta))$ rows of $M$ uniformly at random and independently. 
       			\item For each $i \leq \ell$, let $\hat{C}_i$ be the indices of the columns $j$ such that $M(i,j) \geq \eta^2 \alpha^5/k$.
            %\item Let $\hat{C}_{\ell+1} = [n] \setminus \cup_{i \leq \ell} \hat{C}_i$.
       		
    	\item Choose a uniformly random $S \subseteq [\ell]$ and output $Y_1 = \cup_{i \in S} \hat{C}_i$ and $Y_2 = Y \setminus Y_1$.
    	\end{enumerate}%\textbf{Brute-Force Search Over Partial Clusterings:} For each subset $S \subseteq [\ell+1]$, recursively run two instances of Algorithm~\ref{algo:polynomial-rounding-for-pseudo-distribution-robust} with inputs $\cup_{i \in S} \hat{C}_i$, $\cup_{i \not \in S} \hat{C}_i$ respectively with outlier parameters $\eta + O(k^3\tau)$ for both runs.
    	%\item If either run fails, output fail and return. Otherwise output the union of clusters returned by the two runs of the algorithm.
      \end{enumerate}
    \end{description}
  \end{algorithm}
\end{mdframed}
% \begin{mdframed}
%   \begin{algorithm}[Partial Clustering General Mixtures]
%     \label{algo:rounding-for-pseudo-distribution-robust}\mbox{}
%     \begin{description}
%     \item[Given:]
%         An $\epsilon$-corruption $Y$ of original uncorrupted sample $X = C_1 \cup C_2 \cup \ldots C_k$ with true clusters $C_1, C_2 , \ldots, C_k$.
%     \item[Output:]
%       A partition of $Y$ into an approximately correct clustering $\hat{C}_1, \hat{C}_2, \ldots, \hat{C}_k$.
%     \item[Operation:]\mbox{}
%     \begin{enumerate}
%     \item Find a pseudo-distribution $\tzeta$ satisfying $\cA_{rob}$ minimizing $\Norm{\pE[w]}_2^2$.
%       \item For $M = \pE_{w \sim \tzeta} [ww^{\top}]$, repeat for $1 \leq \ell \leq k$:
%         \begin{enumerate} \item Choose a uniformly random row $i$ of $M$.
%         \item Let $\hat{C}_{\ell}$ be the largest $\frac{n}{k}$ entries in the $i$th row of $M$.
%         \item Remove the rows and columns with indices in $\hat{C}_{\ell}$.
%        \end{enumerate}
%       \end{enumerate}
%     \end{description}
%   \end{algorithm}
% \end{mdframed}

\subsection{Analysis} 

% Our analysis in the following subsections will work assuming that the input sample $X$ (an $\epsilon$-corruption of which 
% is given as input to our algorithms) satisfies some deterministic conditions that we collect together in the definition below. 

% \begin{condition}[Good Sample for Partial Clustering] \label{cond:good-sample-for-clustering}
% A subset $X \subseteq \R^d$ of size $n$ is said to be a good sample from a mixture $\sum_i w_i \cN(\mu_i,\Sigma_i)$ if there exists a partition $X = X_1 \cup X_2 \cup \cdots X_k \subseteq \R^d$ with empirical mean and covariance $\hat{\mu}_1, \hat{\Sigma}_1, \ldots, \hat{\mu}_k, \hat{\Sigma}_k$ such that for all $r \in [k]$ and $s = \poly(k/\eta)$, 
% \begin{enumerate}
%   \item Empirical mean: $\Iprod{\hat{\mu}_r  - \mu(r),v}^2 \leq 0.1 v^{\top} \Sigma(r) v$. % \sqrt{\frac{\trace{\Sigma_{\ell}} }{m_\ell n}} + \sqrt{\frac{\|\Sigma_{\ell}\|_2d}{m_{\ell n}}}$
%   \item Empirical covariance: $ \left(1 - \frac{1}{2^{2s}}\right)\Sigma_r \preceq \hat{\Sigma}_r \preceq \left(1 + \frac{1}{2^{2s}}\right) \Sigma_r$.
%   \item Certifiable Anti-concentration: For all $\tau \geq \poly(\eta/k)$,
%   % \begin{enumerate}
%   %   \item For all $x_i \in C_{\ell}$, \[ \forall v\in \mathbb{R}^d,
%   %     \norm{v}_2^{2t-2} \Iprod{x_i,v}^2 +\gamma_3^2 p^2 (\Iprod{\Sigma_{\ell}^{-\frac{1}{2}} x_i,v})
%   %     \geq \gamma_3^2 \norm{v}_2^{2t}
% %     \]
% \[
% \sststile{2s(\tau)}{v} \Set{
% \frac{1}{|X_r|^2}\sum_{\substack{ i\neq j \in X_r}}  q^2_{\tau, \hat{\Sigma}(r)} \Paren{x_i-x_j,v } \leq 10C\tau \Paren{v^{\top}\hat{\Sigma}(r) v}^{2s}_2}\mcom
% \]

% \[
% \sststile{2s(\tau)}{v} \Set{
% \frac{1}{|X_r||X_{r'}|}\sum_{\substack{ i_1, i_2 \in X_r, j_1, j_2 \in X_{r'}}}  q^2_{\tau, \hat{\Sigma}(r)} \Paren{x_{i_1} -x_{i_2} -x_{j_1} + x_{j_2},v } \leq 10C\tau \Paren{v^{\top}(\hat{\Sigma}(r) + \hat{\Sigma}(r') v}^{2s}_2}\mper
% \]

% \item Certifiable Hypercontractivity: For every $j \leq s$,
% \[
% \sststile{2s}{Q} \Set{
% \frac{k^2}{n^2} \sum_{\substack{ i\neq j \in X_r}}  Q(x_i-x_j)^{2j}
%      \leq (Cj)^{2j} 2^{2j} \Norm{\hat{\Sigma}(r)^{\frac{1}{2}}Q\hat{\Sigma}(r)^{\frac{1}{2}}}_F^{2j}}\mper
% \]
% \end{enumerate}
% \end{condition}

% It is easy to verify using standard concentration arguments (see Section~B of Appendix in~\cite{BK20}) 
% that a large enough sample $X$ from a mixture of $k$ Gaussians is a good sample.

% \begin{fact}[Typical samples are good] \label{lem:typical-samples-good}
% %\Pnote{we are \emph{not} working with GMM models.  See discussion at the beginning of the section. Edited to the version of the statement we need.}
% Let $X = X_1 \cup X_2 \cup \ldots X_k$ be a sample of size $n \geq n_0 = O\Paren{ (s(\poly(\eta/k))d)^{8s(\poly(\eta/k))} k \log k}$ from $\sum_i w_i \cN(\mu_i,\Sigma_i)$. Then, $X$ is good with probability at least $1-1/d$. Furthermore, if there is a pair of components $i,j$ in the mixture such that $\cN(\mu_i,\Sigma_i), \cN(\mu_j,\Sigma_j)$ are $\Delta$-separated in mean distance (spectral distance or relative Frobenius distance, respectively), then $X_i, X_j$ are $\Delta/2$-separated in mean distance (spectral distance or relative Frobenius distance respectively). 
% % Let $\eta>0$ and $\cD$ be a nice distribution. Let $\cluster_{\cD,k}$ be a $\Delta$-separated mixture model, for some $\Delta>1$.
% %Further, the the uniform distribution on  $C_1,C_2,\ldots, C_k$ are pairwise $\Delta/2$-separated.
% \end{fact}

\paragraph{Simultaneous Intersection Bounds.}

The key observation for proving the first theorem is the following lemma 
that gives a sum-of-squares proof that no $z$ that satisfies the constraints $\cup_{i= 1}^5 \cA_i$ 
can have simultaneously large intersections with the $\Delta$-parameter 
separated component Gaussians.


\begin{lemma}[Simultaneous Intersection Bounds for TV-separated case] \label{lem:simultaneous-intersection-bounds}
Let $Y$ be an $\epsilon$-corruption of a sample $X$ of size $n\geq \paren{dk}^{Ct}/\epsilon$ for a large enough constant $C>0$, from $\calM = \sum_i w_i \cN(\mu_i,\Sigma_i)$ satisfying Condition~\ref{cond:convergence-of-moment-tensors} with parameters $t = (k/\eta)^{O(k)}$ and 
$\gamma \leq \epsilon d^{-8t}k^{-Ct}$, for a sufficiently large constant $C>0$.  
Suppose further that $w_i \geq \alpha > 2\epsilon$ for every $i$ and that 
there are $i, j$ such that $\cN(\mu_i,\Sigma_i)$ and $\cN(\mu_j,\Sigma_j)$ 
are $\Delta$-parameter separated for $\Delta = (k/\eta)^{O(k)}$. 
Then, there exists a partition of $[k]$ into $S \cup L$ such that, $|S|, |L| < k$ 
and for $z(X_r) = \frac{1}{\alpha n}\sum_{i \in X_r} z_i$,% \cdot \1 (y_i = x_i)$,  
\[
\cup_{i=1}^5\cA_i \sststile{{(k/\eta \alpha)}^{\poly(k)}}{z} \Set{\sum_{i \in S, j \in L} z(X_i)z(X_{j}) \leq  O(k^2 \epsilon/\alpha) + \eta/\alpha}\mper
\]
\end{lemma}


\noindent The proof of Lemma~\ref{lem:simultaneous-intersection-bounds} is given in 
Section~\ref{ssec:simultaneous-intersection-bounds}.

For the second theorem, we use the following version that strengthens the separation assumption 
and lowers the degree of the sum-of-squares proof (and consequently the running time of the algorithm) as a result.

\begin{lemma}[Simultaneous Intersection Bounds for Frobenius Separated Case] 
\label{lem:simultaneous-intersection-bounds-poly-clustering}
% Let $X$ be a sample of size $n\geq n_0 = d^{(k/\eta)^{O(k)}}$ from a $k$-mixture of 
% Gaussians $\sum_{i} w_i \cN(\mu_i,\Sigma_i)$ with covariance $\Sigma$, 
% and $w_i \geq \alpha$ for each $i$. Suppose there exist $r,r'$ such that 
% $\Norm{\Sigma^{-1/2}(\Sigma_r-\Sigma_{r'})\Sigma^{-1/2}}_F^2 \geq 10^8 k^2 \frac{t^4}{{(\beta \alpha^4)}^{2/t}}$. 
Let $t \in \N$. Let $X$ be a sample of size $n\geq \paren{dk}^{Ct}/\epsilon$ for a large enough constant $C>0$, from 
$\calM = \sum_i w_i \cN(\mu_i,\Sigma_i)$ that satisfies Condition~\ref{cond:convergence-of-moment-tensors} 
with parameters $2t$ and $\gamma \leq \epsilon d^{-8t}k^{-Ck}$, for a large enough constant $C >0$. 
Suppose further that $w_i \geq \alpha > 2 \epsilon$ for each $i \in [k]$, 
and that for some $t \in \N$, $\beta > 0$ there exist $i,j \leq k$ such that 
$\Norm{\Sigma^{\dagger/2}(\Sigma_i -\Sigma_j)\Sigma^{\dagger/2}}_F^2 = \Omega\left((k^2 t^4)/(\beta \alpha^4)^{2/t}\right)$, 
where $\Sigma$ is the covariance of the mixture $\calM$. 
Then, for any $\epsilon$-corruption $Y$ of $X$, there exists a partition of $[k] = S \cup T$ such that  
\[
\cup_{i = 1}^4\cA_i  \sststile{2t}{z} \Set{\sum_{i \in S} \sum_{j\in T} z(X_i) z(X_j) \leq O(k^2)\sqrt{\beta} +O(k^2)\epsilon/\alpha}\mper
\]
\end{lemma}

\noindent The proof of Lemma~\ref{lem:simultaneous-intersection-bounds-poly-clustering} is given in 
Section~\ref{ssec:simultaneous-intersection-bounds-poly-clustering}.


Notice that the main difference between the above two lemmas 
is the constraint systems they use. Specifically, the second lemma does \emph{not} enforce 
certifiable anti-concentration constraints. As a result, there is a difference in 
the degree of the sum-of-squares proofs they claim; the degree of the SoS proof in the second lemma
does not depend on the inverse minimum mixture weight. 

First, we complete the proof of the Theorem~\ref{thm:partial-clustering-non-poly}. 
The proof of Theorem~\ref{thm:partial-clustering-poly} is exactly the same except 
for the use of Lemma~\ref{lem:simultaneous-intersection-bounds-poly-clustering} 
(and thus has the exponent in the running time independent of $1/\alpha$) 
instead of Lemma~\ref{lem:simultaneous-intersection-bounds}.

\begin{proof}[Proof of Theorem~\ref{thm:partial-clustering-non-poly}]

Let $\eta' = O(\eta^2 \alpha^3/k)$. We will prove that whenever $\Delta \geq \poly(k/\eta')^k = \poly(\frac{k}{\eta \alpha})^k$, Algorithm~\ref{algo:robust-partial-clustering}, when  run with input $Y$, with probability at least $0.99$, 
recovers a collection $\hat{C}_1, \hat{C}_2,\ldots, \hat{C}_{\ell}$ of $\ell = O(\frac{1}{\alpha} \log k/\eta)$ 
subsets of indices satisfying $|\cup_{i \leq \ell} \hat{C}_i| \geq (1-\eta'/k^{40})n$ 
such that there is a partition $S \cup L = [\ell]$, $0 < |S| <\ell$ satisfying:
\begin{equation}\label{eq:partial-recovery-clusterwise}
\min\Biggl\{ \frac{1}{\alpha n} |\hat{C}_i \cap \cup_{j \in S} X_j|, \frac{1}{\alpha n} |\hat{C}_i \cap \cup_{j \in L} X_j| \Biggr\} \leq 100 \eta' /\alpha^3 + O(\epsilon/\alpha^4)\mper 
\end{equation}
We first argue that this suffices to complete the proof.
Split $[\ell]$ into two groups $G_S, G_L$ as follows.
For each $i$, let $j = \argmax_{r \in [\ell]} \frac{1}{\alpha n} |\hat{C}_i \cap X_r|$.
If $j \in S$, add it to $G_S$, else add it to $G_L$.
%Observe that this process is well-defined in that we cannot have two distinct maximizers $j, j'$ of $\frac{k}{n} |\hat{C}_i \cap X_r|$ such that $j$ and $j'$ lie in $S,L$ or $L,S$, respectively. This is because our rounding outputs $\hat{C}_i$ that satisfies $\frac{k}{n}  |\hat{C}_i \cap X_r| \geq \frac{k}{n}\cdot \frac{n}{k^2} = \frac{1}{k}$. OTOH, for appropriate  $\eta, \tau$ it follows from by Lemma~\ref{lem:partial-cluster-recovery}, $\min\left\{ \frac{k}{n} |\hat{C}_i \cap \cup_{j \in S} X_j|, \frac{k}{n} |\hat{C}_i \cap \cup_{j \in L} X_j| \right\} < 1/k$, and thus the maximizer must lie in exactly one of $S$ or $L$.
Observe that this process is well-defined - i.e, there cannot be $j\in S$ and $j' \in L$ that both maximize $\frac{1}{\alpha n} |\hat{C}_i \cap X_r|$ as $r$ varies over $[k]$. To see this, WLOG, assume $j \in S$.  Note that $\frac{1}{\alpha n} |\hat{C}_i \cap X_j| \geq 1/k$. Then, we immediately obtain: $\frac{1}{\alpha n} |\cup_{j \in S} X_j \cap \hat{C}_i| \geq 1/k$. Now, if we ensure that $\eta' \leq \alpha^3/k^2$ and $\epsilon \leq O(\alpha^4/k)$, then, $\frac{1}{\alpha n} |\hat{C}_i \cap \cup_{j' \in L} X_{j'}|$ is at most the RHS of \eqref{eq:partial-recovery-clusterwise} which is $\ll 1/k$. This completes the proof of well-definedness. %Combining the last two claims  < \eta/\alpha + O(\epsilon/\alpha) \ll 1/k$. 

% We now show that there is a non-trivial partition of $[\ell]$ into $S$ and $L$ that satisfies the requirements of the theorem. This immediately implies that the algorithm succeeds with probability at least $0.99 \cdot 2^{-\ell} = \alpha^{O(k)}$ as desired. 

% For each $i \in G_S$, we have that $\frac{1}{|\hat{C}_i|} |\hat{C}_i \cap \cup_{j \in L} X_j| \leq \eta' + O(\epsilon/\alpha)$.
Now, adding up \eqref{eq:partial-recovery-clusterwise} for each $i \in S$ yields that $\frac{1}{|\hat{C}_i|} | \Paren{\cup_{i \in G_S} X_i} \cap \cup_{j \in L} X_j| \leq O(\log(k/\eta')/\alpha)  \Paren{\eta' + O(\epsilon/\alpha)}$, 
where we used that $|G_S| \leq \ell$. Combined with $|\cup_{i \leq \ell} \hat{C}_i| \geq (1-\eta'/k^{40})n$, we obtain that $|\cup_{i \in G_S} X_i| \geq 1- \eta'/k^{40} - O(\log(k/\eta')/\alpha)  \Paren{\eta' + O(\epsilon/\alpha)} = \eta + O(\log(k/\eta \alpha)\epsilon/\alpha^2)$ for $\eta' \leq O(\eta^2 \alpha^3/k)$.

We now go ahead and establish \eqref{eq:partial-recovery-clusterwise}. 
Let $\tzeta$ be a pseudo-distribution satisfying $\cA$ of degree $(k/\eta)^{\poly(k)}$ satisfying $\pE_{\tzeta} z_i = \alpha$ for every $i$. Such a pseudo-distribution exists. To see why, let $\tzeta$ be the actual distribution that always sets $X' = X$, chooses an $i$ with probability $w_i$ and outputs a uniformly subset $\hat{C}$ of size $\alpha n$ of $X_i$ conditioned on $\hat{C}$ satisfying $\cA$. Then, notice that since $X$ satisfies Condition~\ref{cond:convergence-of-moment-tensors}, by Fact~\ref{fact:moments-to-analytic-properties}, the uniform distribution on each $X_i$ has $t$-certifiably $C$-hypercontractive degree $2$ polynomials and is $t$-certifiably $C\delta$-anti-concentrated. By an concentration argument using high-order Chebyshev inequality, similar to the proof of Lemma~\ref{lem:det-suffices} (applied to uniform distribution on $X_i$ of size $n \geq (dk)^{O(t)}$, $\hat{C}$ chosen above satisfies the constraints $\cA$ with probability at least $1-o_d(1)$. Observe that the probabililty that $z_i$ is set to $1$ under this distribution is then at most $\alpha+o_d(1)$. Thus, such a distribution satisfies all the constraints in $\cA$. 

Next, let $M = \pE_{\tzeta}[zz^{\top}]$. Then same basic observations as in Chapter 4.3 of~\cite{TCS-086} (see also the proof of Theorem 5.1 in ~\cite{BK20}) yield that:
\begin{enumerate}
  \item $\alpha \geq M(i,j) \geq 0$ for all $i,j$,
  \item $M(i,i) = \alpha$ for all $i$,
  \item $\E_{j \sim [n]} M(i,j) = \alpha^2$ for every $i$.
\end{enumerate}
%Let $\eta' = \eta^2/k^3$, choose $\delta = {\eta'}^3/k^{6}$. 
Call an entry of $M$ large if it exceeds $\alpha^2 \eta'$. For each $i$, let $B_i$ be the set of large entries in row $i$ of $M$. Then, using (3) and (1) above gives that $|B_i| \geq \alpha(1-\alpha\eta')n$ for each $1 \leq  i \leq n$. Next, call a row $i$ ``good'' if $\frac{1}{\alpha n}\min \{ \abs{\cup_{r \in L} X_r \cap B_i}, \abs{\cup_{r' \in S} X_{r'} \cap B_i}\} \leq 100 \eta' /\alpha^3 + O(\epsilon/\alpha^4)$. Let us estimate the fraction of rows of $M$ that are good. 

Towards that goal, let us apply Lemma~\ref{lem:simultaneous-intersection-bounds} with $\eta$ set to $\eta'$ and use Fact~\ref{fact:sos-completeness} (SoS Completeness),  to obtain $\sum_{r \in S, r' \in L}\E_{i \in X_r} \E_{j \in X_{r'}} M(i,j)  \leq \eta' +O(\epsilon/\alpha)$. Using Markov's inequality, with probability $1-\alpha^3/100$ over the uniformly random choice of $i$, $\E_{ j \in X_{r'}} M(i,j) \leq 100 \frac{1}{\alpha^3}\eta' + O(\epsilon/\alpha^4)$. Thus, $1-\alpha^3/100$ fraction of the rows of $M$ are good.

Next, let $R$ be the set of $\frac{100}{\alpha} \log \frac{k^{50}}{\eta'}$ rows sampled in the run of the algorithm and set $\hat{C}_i = B_i$ for every $i \in R$. The probability that all of them are good is then at least $(1-\alpha^3/100)^{\frac{100}{\alpha} \log \frac{k^{50}}{\alpha \eta'}} \geq 1-\alpha$. Let us estimate the probability that $|\cup_{i \in R} \hat{C}_i| \geq (1-\eta'/k^{40})n$. For a uniformly random $i$, the chance that a given point $t \in B_i$ is at least $\alpha(1-\alpha \eta')$. Thus, the chance that $t \not \in \cup_{i \in R}B_i$ is at most $(1-\alpha/2)^{100/\alpha \log k^{50}/(\alpha \eta')} \leq \eta'/k^{50}$. Thus, the expected number of $t$ that are not covered by $\cup_{i \in R} \hat{C}_i$ is at most $n \eta' /k^{50}$. Thus, by Markov's inequality, with probability at least $1-1/k^{10}$, $1-\eta'/k^{40}$ fraction of $t$ are covered in $\cup_{i \in R} \hat{C}_i$. By the above computations and a union bound, with probability at least $1-\eta'/k^{10}$ both the conditions below hold simultaneously: 1) each of the $\frac{100}{\alpha} \log k^{50}/\eta'$ rows $R$ sampled are good and 2) $|\cup_{i \in R} \hat{C}_i| \geq (1-\eta'/k^{40})n$.  This completes the proof.
\end{proof}

%Let's now condition on the events that   Let $\hat{C}_{\ell+1} =[n] \setminus \cup_{i \leq \ell} \hat{C}_i$ be the set of indices that are not covered in $\cup_{i \in R} \hat{C}_i$. Then, $\cup_{i \leq \ell+1} \hat{C}_i$ covers all points in $[n]$.

% We will show that the following way of grouping this partition into two buckets: $R_L = R \cap \cup_{i \in L} X_i$ and $R_S = R \setminus R_L$ satisfies the requirements of the lemma. To see this, note that $\abs{\cup_{i \in R_L} \hat{C}_i \cap \cup_{i \in S} X_i} \leq n/k 100 k^3 \eta' +O(k^3\tau)$. Similarly, $\abs{\cup_{i \in R_S} \hat{C}_i \cup P \cap \cup_{i \in L} X_i} \leq n/k 100 k^3 \eta' + |P| \leq n/k (100 k^3 \eta' + \eta' k^{-40})+ O(k^3\tau)$. 

% Choosing $\eta' \leq \eta/k^{10}$ completes the proof. 


\subsection{Proof of Lemma~\ref{lem:simultaneous-intersection-bounds}} \label{ssec:simultaneous-intersection-bounds}
% Our analysis will rely on the following simultaneous proxy intersection bounds from \cite{BK20}. Informally, the following two results say that there is a partition of the unknown clusters into two groups such that any solution $z$ to the constraint system above cannot simultaneously have a large intersection with cluster pairs that cross the partition. The methodology of the proof is largely based on the ideas in~\cite{BK20} and the first lemma follows directly by a slight modification of the analysis of the partial clustering algorithm in~\cite{BK20}.

Our proof is based on the following simultaneous intersection bounds from~\cite{BK20}. 
We will use the following lemma that forms the crux of the analysis of the clustering algorithm in~\cite{BK20}:

\begin{lemma}[Simultaneous Intersection Bounds, Lemma~5.4 in~\cite{BK20}] \label{lem:intersection-bounds-non-poly}
Fix $\delta >0, k \in \N$. Let $X = X_1 \cup X_2 \cup \ldots X_k$ be a good sample of size $n$ from a $k$-mixture 
$\sum_i w_i \cN(\mu_i,\Sigma_i)$ of Gaussians. Let $Y$ be any $\epsilon$-corruption of $X$. 
Suppose there are $r,r' \leq k$ such that one of the following three conditions hold for some $\Delta \geq (k/\delta)^{O(k)}$:
\begin{enumerate}
\item there exists a $v$ such that $v^{\top}\Sigma(r') v > \Delta v^{\top}\Sigma(r') v$ and 
$B = \max_{i \leq k} \frac{v^{\top} \Sigma(i)v}{v^{\top}\Sigma(r')v}$, or 

\item there exists a $v \in \R^d$ such that $\Iprod{\mu(r) -\mu(r'),v}_2^2 \geq \Delta^2 v^{\top} \Paren{\Sigma(r) +\Sigma(r')} v$, or, 

\item $\Norm{\Sigma(r')^{-1/2}\Sigma(r)\Sigma(r')^{-1/2} - I}_F^2 \geq 
\Delta^2 \Paren{ \Norm{\Sigma(r')^{-1/2}\Sigma(r)^{1/2}}_{\mathrm{op}}^4}$.
\end{enumerate}
Then, for the linear polynomial $z(X_r) = \frac{1}{\alpha n} \sum_{i \in X_r} z_i$ in indeterminates $z_i$s satisfies:
\[
\cup_{i \leq 5} \cA_i \sststile{(k/\delta)^{O(k)}\log (2B)}{z} \Set{z(X_r)z(X_{r'}) \leq  O(\sqrt{\delta}) + O(\epsilon/\alpha) }\mper
\]
\end{lemma}



% \begin{lemma}[Simultaneous Intersection Bounds]\label{lem:intersection-bounds-from-spectral-separation-robust}


% Suppose there exists a $v$ such that $v^{\top}\Sigma(r') v > \Delta_{\spe} v^{\top}\Sigma(r') v$. Let $z'(X_r) = \sum_{i\in X_r: y_i = x_i} z(i)$ for each $r \leq k$. Let $B = \max_{i \leq k} \frac{v^{\top} \Sigma(i)v}{v^{\top}\Sigma(r')v}$.

% Then, whenever $\Delta_{\spe} \gg Cs/\delta$, 
% \[
% \cup_{i \leq 5} \cA_i \sststile{O(s\log (2B))}{z} \Set{z'(X_r)z'(X_{r'}) \leq  O(\sqrt{\delta}) + O(\epsilon/\alpha) }\mper
% \]
% \end{lemma}


% \begin{lemma}[Simultaneous Proxy Intersection Bounds from Mean Separation (Lemma 5.15)]\label{lem:intersection-bounds-from-mean-separation-robust}
% Suppose there exists a $v \in \R^d$ such that $\Iprod{\mu(r) -\mu(r'),v}_2^2 \geq \Delta^2_m v^{\top} \Paren{\Sigma(r) +\Sigma(r')} v$. 

% Then, whenever $\Delta_m \gg Cs/\delta$, 
% \[
% \cup_{i \leq 5} \cA_i \sststile{O(s\log  \kappa)}{z} \Set{z'(X_r)z'(X_{r'}) \leq  O(\sqrt{\delta}) +O(\epsilon/\alpha) }\mper
% \]

% \end{lemma}




% \begin{lemma}[Simultaneous Proxy Intersection Bounds from Relative Frobenius Separation (Lemma 5.16)]
% Suppose $\Norm{\Sigma(r')^{-1/2}\Sigma(r)\Sigma(r')^{-1/2} - I}_F^2 \geq \Delta_{cov}^2 \Paren{ \Norm{\Sigma(r')^{-1/2}\Sigma(r)^{1/2}}_{op}^4}$ for $\Delta_{cov} \gg C/\delta^2$. Then, 
% \[
% \cup_{i \leq 5} \cA_i \sststile{O(s\log \kappa)}{z} \Set{z'(X_r) z'(X_{r'}) \leq O(\delta^{1/3}) + O(\epsilon/\alpha)}\mper
% \]
%  \label{lem:intersection-bounds-from-rel-frob-sep-robust}
% \end{lemma}

% \begin{lemma}[Simultaneous Intersections Bounds Across Bipartition, Spectral Separation Case] \label{lem:sim-intersection-bipartition-bound}
% Suppose there exists a direction $v$ such that $\Delta v^{\top}\Sigma_1 v \leq v^{\top}\Sigma_2v$ for some $\Delta \geq \poly(k/\eta)^k$. Then, 
% There exists a partition $S \cup L =[k]$ such that $|S| < k$ satisfying:
% \[
% \cA \sststile{}{} \Set{ \sum_{r \in S, r' \in L} z(X_r) z(X_{r'}) \leq  \eta + O(\epsilon/\alpha) }\mper
% \]
% \end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:simultaneous-intersection-bounds}]
Without loss of generality, assume that the pair of separated components are $\cN(\mu_1,\Sigma_1)$ and $\cN(\mu_2,\Sigma_2)$. Let us start with the case when the pair is spectrally separated. 
Then, there is a $v \in \R^d$ such that $\Delta v^{\top} \Sigma_1v \leq v^{\top} \Sigma_k v$. 

Consider an ordering of the true clusters along the direction $v$, renaming cluster indices if needed, such that $v^{\top} \Sigma(1) v \leq v^{\top}\Sigma(2)v \leq \ldots v^{\top}\Sigma(k)v$. Let $j \leq k'$ be the largest integer such that $\poly(k/\eta)v^{\top}\Sigma(j)v \leq v^{\top}\Sigma(j+1)v$. Further, observe that since $j$ is defined to be the largest index which incurs separation $\poly(k/\eta)$, all indices in $[j,k]$ have spectral bound at most $\poly(k/\eta)$ and thus $\frac{v^{\top} \Sigma(k)v}{v^{\top}\Sigma(j)v} \leq \poly(k/\eta)^{k}$.

% \textbf{Case 1}: No pair of clusters $X_{r},X_{r'}$ is spectrally separated.
% In this case, for every direction $v$, either $v^{\top} \Sigma(i) v = 0$ for all $i \leq k'$ or $\frac{v^{\top} \Sigma(r) v}{v^{\top} \Sigma(r') v} \leq \Delta \leq O(s(\poly(\eta/k))^k)$ for all $r,r'$. Thus, in particular, the spread $\kappa \leq \Delta$. Applying Lemma~\ref{lem:intersection-bounds-from-separation-robust} and plugging in the upper bound on $\kappa$ immediately yields that for every $1 \leq r < r' \leq k'$
% \[
% \cA \sststile{O( {k'}^2 s^2 \poly \log (s))}{w} \Set{\sum_{r \neq r'} w(X_r) w(X_{r'}) \leq O(k'\tau) + \eta}\mper
% \]

% Thus, in this case, we recover every cluster approximately and thus can set $S$ and $L$ to be any non-trivial partition (that is, both $S$ and $L$ are non-empty) and finish the proof. 

 
Applying Lemma~\ref{lem:intersection-bounds-non-poly} with the above direction $v$ to every $r <j$ and $r' \geq j$ and observing that the parameter $B$ in each case is at most $\frac{v^{\top} \Sigma(k)v}{v^{\top}\Sigma(j)v} \leq \Delta^{k}$ yields:

\[
\cA \sststile{ O({k}^2 s^2 \poly \log (\Delta) )}{} \Set{z(X_r)z(X_{r'}) \leq O(\epsilon/\alpha) +\sqrt{\delta}}\mper
\]

Adding up the above inequalities over all $r \leq j-1$ and $r' \geq j+1$ and taking $S = [j-1]$, $T = [k]\setminus [j-1]$ completes the proof in this case. 

Next, let us take the case when $\cN(\mu_1,\Sigma_1)$ and $\cN(\mu_2,\Sigma_2)$ are mean-separated. WLOG, suppose $\langle \mu_1,v \rangle \leq \langle \mu_2, v \rangle \ldots \leq \langle \mu_k, v\rangle$. Then, we know that $\langle \mu_k-\mu_1, v \rangle \geq \Delta v^{\top} \Sigma_i v$. Thus, there must exist an $i$ such that $\langle \mu_i - \mu_{i+1},v \rangle \geq \Delta v^{\top} \Sigma_i v/k$. Let $S = [i]$ and $L= [k] \setminus S$. Applying Lemma~\ref{lem:intersection-bounds-from-mean-separation-robust} and arguing as in the previous lemma (and noting that $\kappa = \poly(k)$) completes the proof.

Finally, let us work with the case of relative Frobenius separation. Since $\|\Sigma_1^{-1/2}\Sigma_k^{1/2}\| \leq \poly(k)$, the hypothesis implies that $\Norm{\Sigma_1- \Sigma_2}_F \geq \Delta/\poly(k)$. Let $B = \Sigma_1 -\Sigma_2$ and let $A = B/\Norm{B}_F$.
WLOG, suppose $\iprod{\Sigma_1,A}\leq \ldots \iprod{\Sigma_k,A}$.  
Then, since $\iprod{\Sigma_k,A} - \iprod{\Sigma_1,A} \geq \Delta/\poly(k)$, there must exist an $i$ such that $\iprod{\Sigma_{i+1},A} - \iprod{\Sigma_{i},A} \geq \Delta/\poly(k)$. Let us now set $S = [i]$ and $L = [k] \setminus S$. 

Then, for every $i \in S$ and $j \in L$, we must have: $\iprod{\Sigma_j,A} - \iprod{\Sigma_i,A}\geq \Delta/\poly(k)$. 
Thus, $\Norm{\Sigma_j-\Sigma_i}_F \geq \Delta/\poly(k)$. 
And thus, $\Delta/\poly(k)  \leq \Norm{\Sigma_j-\Sigma_i}_F \leq \Norm{\Sigma_i^{-1/2}\Sigma_j^{1/2}}_2^2 \Norm{\Sigma_i^{-1/2}\Sigma_j\Sigma_i^{-1/2}-I}_F$. Rearranging and using the bound on $\Norm{\Sigma_i^{-1/2}\Sigma_j^{1/2}}_2^2$ yields that $\Norm{\Sigma_i^{-1/2}\Sigma_j\Sigma_i^{-1/2}-I}_F \geq \Delta/\poly(k)$. 

A similar argument as in the two cases above now completes the proof.

\end{proof}

% \begin{lemma}[Simultaneous Intersections Bounds Across Bipartition, Mean Separation Case] \label{lem:sim-intersection-bipartition-bound}
% Suppose that for all $v$, $v^{\top}\Sigma_r v \leq k^{O(k)} v^{\top}\Sigma_r' v$ for all $r,r' \leq k$. Suppose further that $\Iprod{\mu_1 - \mu_2,v} \geq \Delta v^{\top} \Sigma_i v$ for all $i$. Then, there exists a partition $S \cup L =[k]$ such that $|S| < k$ satisfying:
% \[
% \cA \sststile{}{} \Set{ \sum_{r \in S, r' \in L} z(X_r) z(X_{r'}) \leq  O(\epsilon/\alpha) + \eta }\mper
% \]
% \end{lemma}

% \begin{proof}

% \end{proof}

% \begin{lemma}[Simultaneous Intersections Bounds Across Bipartition, Frobenius Separation Case] \label{lem:sim-intersection-bipartition-bound}
% Suppose that for all $v$, $v^{\top}\Sigma_r v \leq k^{O(k)} v^{\top}\Sigma_r' v$ for all $r,r' \leq k$. Suppose further that $\Iprod{\mu_i - \mu_j,v} \leq k^{O(k)} \Norm{v}_2$. And finally, suppose that $\Norm{\Sigma_1^{-1/2} \Sigma_k \Sigma_1^{-1/2}-I}_F \geq \Delta$. Then, there exists a partition $S \cup L =[k]$ such that $|S| < k$ satisfying:
% \[
% \cA \sststile{}{} \Set{ \sum_{r \in S, r' \in L} z(X_r) z(X_{r'}) \leq  O(\epsilon/\alpha) + \eta }\mper
% \]
% \end{lemma}
% \begin{proof}

% \end{proof}






% \subsection{Algorithm}
% Covariance constraints introduce a matrix valued indeterminate intended to be the square root of $\Sigma$.
% \begin{equation}
% \text{Covariance Constraints: $\cA_1$} = %  \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &
%       &\Pi
%       &=UU^{\top}\\
%       % &
%       % &\Theta \Pi = \Pi \Theta
%       % &= I\\
%       &
%       &\Pi^2
%       &=\Sigma\\
%       % &
%       % &\Theta^2\Sigma  = \Sigma \Theta^2
%       % &=\Theta\Sigma\Theta =I\\
%     \end{aligned}
%   \right \}
% \end{equation}
% The intersection constraints force that $X'$ be close to $X$. 
% \begin{equation}
% \text{Intersection Constraints: $\cA_2$} = %  \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &\forall i\in [n],
%       & m_i^2
%       & = m_i\\
%       &&
%       \textstyle\sum_{i\in[n]} m_i 
%       &= (1-\epsilon) n\\
%       &\forall i \in [n],
%       &m_i (y_i-x'_i)
%       &= 0
%     \end{aligned}
%   \right \}
% \end{equation}
% The subset constraints introduce $w$, which indicates the subset $\hat{C}$ intended to be the true clusters of $X'$.
% \begin{equation}
% \text{Subset Constraints: $\cA_3$} = %  \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &\forall i\in [n].
%       & w_i^2
%       & = w_i\\
%       &&
%       \textstyle\sum_{i\in[n]} w_i 
%       &= pn\\
%     \end{aligned}
%   \right \}
% \end{equation}

% Parameter constraints create indeterminates to stand for the covariance $\Sigma$ and mean $\mu$ of $\hat{C}$ (indicated by $w$).
% \begin{equation}
% \text{Parameter Constraints: $\cA_4$} = %  \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &
%       &\frac{1}{pn}\sum_{i = 1}^n w_i \Paren{x'_i-\mu}\Paren{x'_i-\mu}^{\top}
%       &= \Sigma\\
%       &
%       &\frac{1}{pn}\sum_{i = 1}^n w_i x'_i
%       &= \mu\\
%     \end{aligned}
%   \right \}
% \end{equation}

%       % &
%       % &\frac{1}{n}\sum_{i = 1}^n w_i x_ix_i^{\top}
%       % &= \Sigma\\
%       % &
%       % &\frac{1}{n}\sum_{i = 1}^n w_i x_i
%       % &= \mu\\


% % Finally, we enforce certifiable anti-concentration and hypercontractivity of $\hat{C}$. 
% % \begin{equation}
% % \text{Certifiable Anti-Concentration : $\cA_4$} =% \cA_{w,\Pi}\colon
% %   \left \{
% %     \begin{aligned}
% %       % &\forall i,j\in [n].
% %       % & w_i w_j \Paren{\norm{v}_2^{2t-2} \Iprod{\Paren{\frac{x_i-x_j}{\sqrt{2}}},v}^2 +\delta^2 p^2 (\Iprod{\Theta \Paren{\frac{x_i-x_j}{\sqrt{2}}},,v})}
% %       % &\geq w_i w_j \Paren{\delta^2 \norm{v}_2^{2t}}\\
% %       &
% %       &\frac{1}{p^2n^2}\sum_{i,j=  1}^n w_i w_j q_{\delta,\Sigma}^2\left(\Paren{x'_i-x'_j},v\right)
% %       &\leq 2^{s(\delta)} C\delta \Paren{v^{\top}\Sigma v}^{s(\delta)}\\
% %       &
% %       &\frac{1}{p^2n^2}\sum_{i,j=  1}^n w_i w_j q_{\tau,\Sigma}^2\left(\Paren{x'_i-x'_j},v\right)
% %       &\leq 2^{s(\tau)} C\tau \Paren{v^{\top}\Sigma v}^{s(\eta)}\\
% %      \end{aligned}
% %     \right\}
% %  \end{equation}

% \begin{equation}
% \text{Mixture Parameters : $\cA_4$} = % \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%      &\forall j \leq 2s
%      &\frac{1}{p^2 n^2} \sum_{i,j \leq n} w_i w_j (x_i'-x_j')(x_i'-x_j')^{\top}
%      &=\Sigma\\
%      &
%      &0.99 I\preceq \Sigma
%      &\preceq 1.01 I
%     \end{aligned}
%   \right \}
% \end{equation}

% \begin{equation}
% \text{Certifiable Hypercontractivity : $\cA_5$} = % \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%      &\forall j \leq 2s
%      &\frac{1}{p^2n^2} \sum_{i,j \leq n} w_i w_j Q(x'_i-x'_j)^{2j}
%      &\leq (Cj)^{2j}2^{2j}\Norm{\Pi Q \Pi}_F^{2j}
%     \end{aligned}
%   \right \}
% \end{equation}

% Our rounding algorithm is exactly the same as in the previous section giving us:
% \begin{mdframed}
%   \begin{algorithm}[Partial Clustering]
%     \label{algo:robust-partial-clustering}\mbox{}
%     \begin{description}
%     \item[Given:]
%         A sample $Y$ of size $n$ for $j \in [k]$. A outlier parameter $\tau > 0$ and an accuracy parameter $\eta > 0$. 
%     \item[Output:]
%       A partition of $Y$ into partial clustering $Y_1 \cup Y_2$.
%     \item[Operation:]\mbox{}
%     \begin{enumerate}
%       %\item \textbf{Base Case:} If $|Y'| = n/k$, accept if Algorithm~\ref{algo:verification-subroutine} applies to $Y'$ with outlier parameter $\tau$ accepts. Otherwise output fail.
%       \item \textbf{SDP Solving:} Find a pseudo-distribution $\tzeta$ satisfying $\cA_{rob}$ minimizing $\Norm{\pE[w]}_2^2$ with number of components set to $j$ and outlier parameter set to $\tau$. If no such pseudo-distribution exists, output fail.
%         \item \textbf{Rounding:} Let $M = \pE_{w \sim \tzeta} [ww^{\top}]$. 
%           \begin{enumerate} \item Choose a uniformly random row $i$ of $M$.
%             \item Choose $\ell = 100 k \log k$ rows of $M$ uniformly at random and independently. 
%             \item For each $i \leq \ell$, let $\hat{C}_i$ be the indices of the columns $j$ such that $M(i,j) \geq \eta/\poly(k)$.
%             \item Let $\hat{C}_{\ell+1} = [n] \setminus \cup_{i \leq \ell} \hat{C}_i$.
%           \end{enumerate}
%       \item Choose a uniformly random $S \subseteq [\ell]$ and output $Y_1 = \cup_{i \in S} \hat{C}_i$ and $Y_2 = Y \setminus Y_1$.%\textbf{Brute-Force Search Over Partial Clusterings:} For each subset $S \subseteq [\ell+1]$, recursively run two instances of Algorithm~\ref{algo:polynomial-rounding-for-pseudo-distribution-robust} with inputs $\cup_{i \in S} \hat{C}_i$, $\cup_{i \not \in S} \hat{C}_i$ respectively with outlier parameters $\eta + O(k^3\tau)$ for both runs.
%       %\item If either run fails, output fail and return. Otherwise output the union of clusters returned by the two runs of the algorithm.
%       \end{enumerate}
%     \end{description}
%   \end{algorithm}
% \end{mdframed}


\subsection{Proof of Lemma~\ref{lem:simultaneous-intersection-bounds-poly-clustering}} 
\label{ssec:simultaneous-intersection-bounds-poly-clustering}

We use $\E_z$ as a shorthand for $\sum_{i = 1}^n z_i$. We will write $\frac{1}{w_r n} \sum_{j \in X_r} z_j = z(X_r)$. 
Note that $z(X_r) \in [0,1]$. 

We will use the following technical facts in the proof:

\begin{fact}[Lower Bounding Sums, Fact 4.19~\cite{BK20}] \label{fact:lower-bounding-sums-SoS}
Let $A,B,C,D$ be scalar-valued indeterminates. Then, for any $\tau >0$,
\[
\Set{0 \leq A, B \leq A+B \leq 1} \cup \Set{0\leq C,D} \cup \Set{C+D\geq \tau} \sststile{2}{A,B,C,D} \Set{ AC+ BD \geq \tau AB}\mper
\]

\end{fact}


\begin{fact}[Cancellation within SoS, Lemma 9.2 in~\cite{BK20}] \label{fact:cancellation-within-sos-constant-rhs}
For indeterminate $a$ and any $t \in \N$, 

\[
\Set{a^{2t} \leq 1} \sststile{2t}{a} \Set{ a\leq 1}\mper
\]
\end{fact}



% \begin{lemma}[Upper Bound on Variance of Degree 2 Polynomials] \label{lem:variance-w-upper-bound}
% For a $d \times d$ matrix valued indeterminate $Q$.  
% \[
% \cA \sststile{4}{Q} \Set{ \E (Q-\E_z Q)^2 \leq 2C/\alpha^2 \Norm{\Sigma^{1/2}Q\Sigma^{1/2}}_F^2 } \mper
% \]
% \end{lemma}

% \begin{proof}
% $X$ is a sample of size $n \geq n_0 = O(d^{4}/\epsilon^2)$ from $\sum_i w_i \cN(\mu_i,\Sigma_i)$. From Fact~\ref{fact:subgaussianity-of-mixtures}, $\sum_i w_i \cN(\mu_i,\Sigma_i)$ is $4$-certifiably $C/\alpha$-subgaussian. Thus, the uniform distribution on $X$ is $4$-certifiably $2C/\alpha$-subgaussian with probability at least $0.99$. 

% We have:
% \[
% \frac{1}{\alpha n} \sum_i z_i (Q(x_i) - \E_w Q)^2 \leq \frac{1}{\alpha n} \sum_i (Q(x_i)- 1/n\sum_i Q_i)^2 \leq 1/\alpha (2C/\alpha-1) \Norm{\Sigma^{1/2} Q \Sigma^{1/2}}_F^2\mcom
% \]
% where we used that $\Sigma$ is the covariance of $\sum_i w_i \cN(\mu_i,\Sigma_i)$. Applying Fact~\ref{fact:mean-variance-subgaussian} completes the proof.

% \end{proof}

\begin{lemma}[Lower-Bound on Variance of Degree 2 Polynomials] \label{lem:lower-bound-variance}
Let $Q \in \R^{d \times d}$. Then, for any $i,j \leq k$,  and $z(X_r) = \frac{1}{\alpha n} \sum_{i \in X_r} z_i $, we have:
\begin{align*}
\cA \sststile{4}{z} \Biggl\{z(X_r)^2 z(X_r')^2 \leq  \frac{(32Ct)^{2t}}{(\E_{X_r} Q - \E_{X_{r'}}Q)^{2t}}  & \Biggl(\frac{\alpha^4}{w_r^2 w_{r'}^2}  \Paren{\E_z (Q-\E_z Q)^{2}}^{t} \\
&+ \frac{\alpha^2}{w_r^2} \Paren{\E_{X_{r'}} (Q-\E_{X_{r'}}Q)^{2}}^t + \frac{\alpha^2}{w_{r'}^2} \Paren{\E_{X_r}(Q-\E_{X_r}Q)^{2}}^t\Biggr)\Biggr\}\mper
\end{align*}
\end{lemma}
\begin{proof}
 
\begin{align*}
\cA \sststile{4}{z} \Biggl\{ \E_z (Q-\E_z Q)^{2t} &= \frac{1}{\alpha^2 n^2} \sum_{i, j \leq n } z_i z_j \Paren{Q(x_i - x_j)- \E_z Q}^{2t} \geq \frac{1}{\alpha^2 n^2} \sum_{i, j \in X_r \text{ or } i,j \in X_{r'}} z_i z_j \Paren{Q(x_i - x_j)- \E_z Q}^{2t}\\
& \geq \frac{1}{2^{2t}} \frac{1}{\alpha^2 n^2} \sum_{i, j \in X_r } z_i z_j \Paren{\E_{X_r}Q -\E_z Q}^{2t} - \frac{1}{\alpha^2n^2} \sum_{i, j \in X_r } w_i w_j \Paren{Q(x_i - x_j)- \E_{X_r}Q}^{2t}\\
&+ \frac{1}{2^{2t}}\frac{1}{\alpha^2 n^2} \sum_{i, j \in  X_r } z_i z_j \Paren{\E_{X_{r'}}Q- \E_z Q}^{2t}-  \frac{1}{\alpha^2 n^2} \sum_{i, j \in  X_{r'} } z_i z_j \Paren{Q(x_i - x_j)- \E_{X_{r'}}Q}^{2t}\\
&= 2^{-2t} (w_r/\alpha)^2 z(X_r)^2 \Paren{\E_{X_r}Q -\E_z Q}^{2t} - \frac{1}{\alpha^2 n^2} \sum_{i, j \in  X_r } \Paren{Q(x_i - x_j)- \E_{X_r}Q}^{2t}\\
&+ 2^{-2t}(w_{r'}/\alpha)^2 z(X_{r'})^2 \Paren{\E_{X_{r'}}Q- \E_z Q}^{2t}- \frac{1}{\alpha^2 n^2} \sum_{i, j \in  X_{r'} } \Paren{Q(x_i - x_j)- \E_{X_{r'}}Q}^{2t}\\
&\geq 2^{-6t} \frac{w_r^2 w_{r'}^2}{\alpha^4} z(X_{r})^2z^2(X_{r'}) (\E_{X_r}Q-\E_{X_{r'}}Q)^{2t} -  (w_r/\alpha)^2  \E_{X_r} (Q-\E_{X_r}Q)^{2t} \\&-
 (w_{r'}/\alpha)^2  \E_{X_{r'}} (Q-\E_{X_{r'}}Q)^{2t}\\
 &\geq 2^{-6t} \frac{w_r^2 w_{r'}^2}{\alpha^4} z(X_{r})^2z^2(X_{r'}) (\E_{X_r}Q-\E_{X_{r'}}Q)^{2t} - (w_r/\alpha)^2 (Ct)^{2t}\Paren{\E_{X_r} (Q-\E_{X_r}Q)^{2}}^t\\
&- (w_{r'}/\alpha)^2  (Ct)^{2t}\Paren{\E_{X_{r'}} (Q-\E_{X_{r'}}Q)^{2}}^t
\Biggr\}\mper
\end{align*}
In the above, we used the almost triangle inequality (Fact~\ref{fact:almost-triangle-sos}) in the first inequality, Fact~\ref{fact:lower-bounding-sums-SoS} in the second inequality and certifiable hypercontractivity constraints in $\cA$ in the last inequality. 
Rearranging completes the proof.
\end{proof}

We can use the lemma above to obtain a simultaneous intersection bound guarantee when there are relative Frobenius separated components in the mixture. 
\begin{lemma} \label{lem:pair-rel-frob}
Suppose $\Norm{\Sigma^{-1/2}(\Sigma_r-\Sigma_{r'})\Sigma^{-1/2}}_F^2 \geq 10^8 \frac{C^6 t^4}{{(\beta \alpha^4)}^{2/t}}$. Then, for $z'(X_r) = \frac{1}{\alpha n} \sum_{i \in X_r} z_i \cdot \1(y_i = x_i)$,  
\[
\cA \sststile{2t}{w} \Set{z'(X_r) z'(X_r') \leq \sqrt{\beta}}\mper
\]
\end{lemma}
\begin{proof}
We work with the transformation $x_i \rightarrow \Sigma^{-1/2}x_i$. Let $\Sigma_z' = \Sigma^{-1/2}\Sigma_z \Sigma^{-1/2}$, $\Sigma_r' = \Sigma^{-1/2} \Sigma_r\Sigma^{-1/2}$ and $\Sigma_{r'}' =\Sigma^{-1/2}\Sigma_{r'}\Sigma^{-1/2}$ be the transformed covariances. Note that transformation is only for the purpose of the argument - our constraint system does not depend on $\Sigma$.

Notice that $\Norm{\Sigma_{r'}'}_2 \leq \frac{1}{w_r}$ and $\Norm{\Sigma_{r'}'}_2 \leq \frac{1}{w_{r'}}$. 


We now apply Lemma~\ref{lem:lower-bound-variance} with $Q = \Sigma_{r}'-\Sigma_{r'}'$. Then, notice that $\E_{X_r}Q - \E_{X_{r'}} Q = \Norm{\Sigma_r' - \Sigma_{r'}'}_F^2 = \Norm{Q}_F^2$. Then, we obtain:

\begin{multline}\label{eq:basic-bound}
\cA \sststile{2t}{z} \Biggl\{z'(X_r)^2 z'(X_r')^2 \\\leq \Paren{\frac{32Ct}{\E_{X_r} Q - \E_{X_{r'}}Q}}^{2t}  \Paren{\frac{\alpha^4}{w_r^2 w_{r'}^2} \Paren{\E_z (Q-\E_z Q)^2}^t + \frac{\alpha^2}{w_r^2} \Paren{\E_{X_{r'}} (Q-\E_{X_{r'}}Q)^2}^t + \frac{\alpha^2}{w_{r'}^2} \Paren{\E_{X_r}(Q-\E_{X_r}Q)^2}}^t\Biggr\}\mper
\end{multline}

\nnnew{Since $X_{r}$ and $X_{r'}$ have certifiably $C$-bounded variance polynomials for $C = 4$ (as a consequence of Condition~\ref{cond:convergence-of-moment-tensors} and Fact~\ref{fact:moments-to-analytic-properties} followed by an application of Lemma~\ref{lem:frob-of-product}), we have:}
\[
\cA \sststile{2}{Q} \Set{\E_{X_{r'}} (Q-\E_{X_{r'}}Q)^2 \leq \nnnew{6\Norm{{\Sigma_{r'}'}^{1/2}Q{\Sigma_{r'}'}^{1/2}}_F^2} \leq \frac{6}{w_{r'}^2} \Norm{Q}_F^2} \;,
\]
and
\[
\cA \sststile{2}{Q} \Set{\E_{X_{r}} (Q-\E_{X_{r}}Q)^2 \leq \nnnew{6\Norm{{\Sigma_{r}'}^{1/2}Q{\Sigma_{r}'}^{1/2}}_F^2} \leq \frac{6}{w_{r}^2} \Norm{Q}_F^2} \mper
\]
Finally, using the bounded-variance constraints in $\cA$, we have: 
\[
\cA \sststile{4}{Q,z} \E (Q-\E_z Q)^2 \leq 6\Norm{Q}_F^2\mper
\]

Plugging these estimates back in \eqref{eq:basic-bound} yields:
\begin{equation}\label{eq:final-bound}
\cA \sststile{4}{z} \Set{z'(X_r)^2 z'(X_r')^2 \leq \frac{(1000Ct)^{2t}}{\Norm{Q}_F^{2t}} \Paren{\frac{2Ct\alpha^2}{w_r^2 w_{r'}^2}} + \frac{\alpha^2}{w_{r'}^2w_r^2}  + \frac{\alpha^2}{w_r^2 w_{r'}^2} =\frac{(2C+2)\alpha^2}{w_r^2 w_{r'}^2} \frac{(1000Ct)^{2t}}{\Norm{Q}_F^{2t}}\leq \frac{(2C+2)(1000Ct)^{2t}}{\alpha^2 \Norm{Q}_F^{2t}}} \mper
\end{equation}

Plugging in the lower bound on $\Norm{Q}_F^{2t}$ and applying Fact~\ref{fact:cancellation-within-sos-constant-rhs} completes the proof. 
\end{proof}

Observe that for $z'(X_r) = \frac{1}{\alpha n}\sum_{i \in X_r} z_i \1(y_i = x_i)$, using that $\Set{z_i^2=z_i}\sststile{2}{z} \Set{z_i \leq 1}$, we have (as in the proof of proxy intersections bounds in Section 5 of ~\cite{BK20}):
$\cA \sststile{2}{z} \Set{z(X_r) = \frac{1}{\alpha n}\sum_{i \in X_r} z_i (\1(y_i = x_i)+(1-\1(y_i=x_i))) \leq  z'(X_r)+ \frac{1}{\alpha n}\sum_{i \leq [n]} (1-\1(y_i=x_i)) = z'(X_r) + \epsilon/\alpha}$. Thus, we immediately obtain:




\begin{corollary}[Proxy Intersection Bounds] \label{cor:rel-frob-poly-clustering}
Suppose $\Norm{\Sigma^{-1/2}(\Sigma_r-\Sigma_{r'})\Sigma^{-1/2}}_F^2 \geq 10^8 \frac{C^6 t^4}{{(\beta p^4)}^{2/t}}$. Then, for $z(X_r) = \frac{1}{\alpha n} \sum_{i \in X_r} z_i$,  
\[
\cA \sststile{2t}{w} \Set{z(X_r) z(X_{r'}) \leq \sqrt{\beta} + O(\epsilon/\alpha)}\mper
\]
\end{corollary}


We can use the above lemma to complete the proof of Lemma~\ref{lem:simultaneous-intersection-bounds-poly-clustering}:




\begin{proof}[Proof of Lemma~\ref{lem:simultaneous-intersection-bounds-poly-clustering}]
WLOG, assume that $\Sigma = I$. 
Let $Q = \Sigma_r - \Sigma_{r'}$ and let $\bar{Q}= Q/\Norm{Q}_F$.
Consider the numbers $v_i = \tr(\Sigma_r \cdot Q)$. 
Then, we know that $\max_{i,j} |v_i - v_j| \geq \Norm{Q}_F$. 
Thus, there must exist a partition of $[k] = S \cup T$ such that $|v_i -v_j| \geq \Norm{Q}_F/k$ whenever $i \in S$ and $j \in T$. 
 
Thus, for every $i \in S$  and $j \in T$, $\Norm{\Sigma_i - \Sigma_j}^2_F \geq \Norm{Q}^2_F/k^2 = 10^8\frac{C^6 t^4}{{(\beta \alpha^4)}^{2/t}}$. 
We can now apply Lemma~\ref{cor:rel-frob-poly-clustering} to every $i \in S, j \in T$ and add up the resulting inequalities to finish the proof.



\end{proof}

% The case when there is a pair of mean-separated components (relative to the mixture covariance) is similar:

% \begin{lemma}
% Suppose there exist $r,r'$ such that $\Norm{\Sigma^{-1/2}(\mu_r - \mu_{r'})}_2 \geq k^2 \beta/p^2$. Then, there is a partition of $[k] = S \cup T$ such that 
% \[
% \cA \sststile{}{} \Set{\sum_{i \in S, j \in T} w(X_i) w(X_j) \leq \beta}\mper
% \]
% \end{lemma}
% \begin{proof}
% As before, we can assume that $\Sigma = I$ by a linear transformation of the input points $Y$. 
% Let $\Norm{\mu_r - \mu_{r'}}_2 = \Delta$.
% Let $v = \mu_r - \mu_{r'}$ and let $\bar{v} = v/\norm{v}_2$. 
% Consider the means $\langle \mu_1,v \rangle, \langle \mu_2,v \rangle, \ldots, \langle\mu_k,v \rangle$ of the mixture components projected to the direction $v$. Then, since the max difference between two of these projections is at least $\Delta$, there must be a partition of the means into $S \cup T$ so that for every $i \in S, j \in T$, $\abs{\langle \mu_i, v\rangle - \langle\mu_j,v\rangle} \geq \Delta/k$. Since $v$ is a unit vector, this implies that for every $i \in S, j \in T$, $\Norm{\mu_i - \mu_j}_2 \geq \Delta/k$. 

% For each such $i,j$, let $Q(x) = \langle\mu_i - \mu_j, x\rangle$. 
% Then, notice that $\E_{X_i} Q(x)-\E_{X_j}Q(x) = \Norm{\mu_i -\mu_j}_2^2$, $\E_{w}(Q-\E Q)^2 \leq  2C/p^2\Norm{\mu_i -\mu_j}_2^2$, and $\E_{X_i} (Q-\E_{X_i} Q)^2 \leq 1/p_i^2, \E_{X_j} (Q-\E_{X_j} Q)^2 \leq 1/p_j^2$.  

% Plugging these bounds in Lemma~\ref{lem:lower-bound-variance}, gives:
% \[
% \cA \sststile{4}{w} \Set{w(X_r)^2 w(X_r')^2 \leq \beta/k^2 }\mper
% \]
% Summing up over all $i\in S, j \in T$ completes the proof.
% \end{proof}


% \begin{corollary}[Simultaneous proxy intersection bounds across a partition]
% Let $Y$ be an $\epsilon$-corrupted sample of size $n\geq n_0 = d^{O(1)}/\alpha$ form a mixture of $k$ Gaussians with weights $w_1, w_2,\ldots, w_k$ and unknown component parameters $\{\mu_i,\Sigma_i\}_{i \leq k}$. Let $\alpha = \min_{i\leq k} w_i$. Suppose further that $\epsilon \ll \alpha$ and that there exist $r,r' \leq k$ such that $\Norm{\Sigma_i -\Sigma_j}_F^2 = \Omega(\frac{t^4}{{(\beta \alpha^4)}^{2/t}})$. Then, there exists a partition of $[k] = S \cup T$ such that:
% \[
% \cA \sststile{2t}{} \Set{ \sum_{i \in S, j \in T} z(X_i)z(X_j) \leq \beta + 2\epsilon/\alpha}\mper
% \] 

% \end{corollary}



\subsection{Special Case: Algorithm for Uniform and Bounded Mixing Weights}
In this subsection, we obtain a polynomial time algorithm when the input mixture has weights that are bounded from below. This includes the case of uniform weights and when the minimum mixing weight is at least some function of $k$. At a high level, our algorithm  partitions the sample into clusters as long as there is a pair of components separated in TV distance and given samples that are not clusterable, runs the tensor decomposition algorithm to list decode. 
We then use standard robust tournament results to pick a hypothesis from the list. 

\begin{theorem}[Robustly Learning Mixtures of Gaussians with Bounded Weights]
\label{thm:robust-GMM-equiweigthed}
Given $0< \epsilon < \bigOk{1}$,
%$0< \epsilon < 1/k^{k^{O(k)}}$ 
let $Y = \{ y_1, y_2, \ldots , y_n\}$ be a multiset of $n \geq n_0=\poly_k\Paren{d, 1/\eps}$ $\epsilon$-corrupted samples 
from a $k$-mixture of Gaussians $\calM =  \sum_{i \leq k} w_i \calN\Paren{\mu_i, \Sigma_i}$, such that $w_i \geq \alpha$. 
Then, there exists an algorithm with running time $\poly_k(n^{1/\alpha} )\cdot\exp\Paren{ \poly_k(1/\alpha,1/\epsilon)}$ 
such that with probability at least $9/10$ it outputs a hypothesis $k$-mixture of Gaussians 
$\widehat{\calM} = \sum_{i \leq k} \hat{w}_i \calN\Paren{\hat{\mu_i}, \hat{\Sigma}_i}$ 
such that $d_{\textrm{TV}}\Paren{\calM, \widehat{\calM}} = \bigOk{\eps}$.  
\end{theorem} 


%\begin{remark}
%For the special case where the input mixture has uniform weights or weights bounded from below by $1/\poly(k)$ or some function of $k$, we obtain an algorithm with running time $\poly_k(n,1/\epsilon)$ that outputs a mixture of $k$ Gaussians which is $\poly_k(\epsilon)$-close to the input mixture.
%\end{remark}

% \begin{mdframed}
%  \begin{algorithm}[Algorithm for Robustly Learning Equi-weighted GMMs]
%    \label{algo:robust-GMM-equi}\mbox{}
%    \begin{description}
%    \item[Input:] An $\epsilon$-corrupted sample $Y = \{y_1, y_2, \ldots, y_n \}$ from a mixture of $k$ Gaussians, $\calM = \sum_{i \in [k]} \frac{1}{k} \cN(\mu_i,\Sigma_i)$. An outlier parameter $\epsilon>0$ and a component-number parameter $k\in \N$.

%    \item[Parameters:]  Let  $c_k=1/(100^k C^{(k+1)!}\mathrm{sf}(k+1)k!)$ be some scalar that only dependent on $k$. For $\ell \in [k]$, let $f_{k,\ell} = \textrm{sf}(k-\ell)/(10^\ell c^{k!/(k-\ell)!}\textrm{sf}(k))$.  

%    \item[Output:] A set of parameter $\{ ( \hat \mu_i, \hat\Sigma_i)\}_{i \leq k}$ such that the mixture $\sum_{i \leq k} \frac{1}{k} \cN(\hat \mu_i, \hat \Sigma_i)$ is $\poly_k(\epsilon)$-close in total variation distance to $\sum_{i \leq k} \frac{1}{k} \cN(\mu_i, \Sigma_i)$. 

%    \item[Operation:]\mbox{}
%    \begin{enumerate}

%   \item \textbf{Clustering via SoS}: Run Algorithm \ref{algo:robust-partial-clustering} with outlier parameter $\epsilon$ and accuracy paramater $\epsilon$. Let $Y_1$ and $Y_2$ be the resulting partition. If $|Y_1| > (1- 2k\epsilon)(n/k)$ recurse by calling Algorithm \ref{algo:robust-partial-clustering}  on $Y_1$ with outlier paramater $k\epsilon$ and similarly with $Y_2$. Let $\tilde{Y}_1 , \tilde{Y}_2, \ldots \tilde{Y}_t$ be the resulting partition for $t \leq k$.
%   %Guess the number of components in $Y_1$ and $Y_2$ to be $k_1$ and $k_2 = k - k_1$ respectively. Recurse, by running Algorithm \ref{algo:robust-GMM-equi} on $Y_1$, with number of components being $k_1$, and the fraction of outliers $\zeta^{1/(100k)}$ and similarly on $Y_2$. Combine the lists obtained from the recursive calls.   
%       \\ \textit{// When the mixture is clusterable, preconditions of Theorem \ref{thm:partial-clustering} are satisfied. The partition is non-trivial and the fraction of outliers goes from $\epsilon \to k \epsilon$. The fraction of outliers in each partition $\tilde{Y}_j$ is $\bigO{k^2\epsilon}$. } 

%       \item For all $j \in [t]$,
%       \begin{enumerate}
%   \item  \textbf{Robust Isotropic Transformation}: Run the algorithm corresponding to Lemma \ref{lem:sampling_from_nearl_isotropic}  on the samples $\tilde{Y}_j$  and let $\hat{\mu}_j,\hat{\Sigma}_j $ be the robust estimates of the mean and covariance. For all $i \in [k]$, apply the affine transformation $y_i \to \hat{\Sigma}_j^{-1/2}\Paren{y_i- \hat{\mu}_j}$ to all samples in $\tilde{Y}_j$.
%  \\ \textit{// The resulting estimates $\hat{\mu}_j, \hat{\Sigma}_j$ satisfy Lemma \ref{lem:sampling_from_nearl_isotropic}, the fraction of outliers. }   
%   \item \textbf{List-Decoding via Tensor Decomposition}:  Run Algorithm \ref{algo:list-recovery-tensor-decomposition} on $\tilde{Y}_j$. Let $\calL_j$ be the resulting list of hypothesis. Concatenate the lists to obtain $\calL$.
%   % For each hypothesis $\{\hat{w}_i, \hat{\mu}_i, \hat{\Sigma}_i \}_{i \in[k]}  \in \calL$ repeat the following: 
%  \\  \textit{// Conditioned on not being clusterable, we satisfy the preconditions of Theorem \ref{thm:list-recovery-by-tensor-decomposition} (see Lemma \ref{lem:list_decoding}). The output is a list that contains $\{\hat{\mu}_i, \hat{\Sigma}_i\}_{i \in [k]}$ s.t.  for all $i \in [k]$, $\Norm{ \hat{\mu}_i - \mu_i }_2 =\bigO{ \gamma^{1/(4c^{k+1}k!)} }$  and $\Norm{ \hat{\Sigma}_i - \Sigma_i }_F =\bigO{\gamma^{1/(4c^{k+1}k!)} } $. }
%     \end{enumerate}
%    \item \textbf{Robust Tournament}: Run a tournament in Lemma~\ref{lem:tournament} over all the hypothesis in $\calL$, and output the winning hypothesis. 
%    \end{enumerate}
   
%    \end{description}
%  \end{algorithm}
% \end{mdframed}

\input{uniform_weights}

==> prelims-sos.tex <==
%!TEX root = main.tex



% The \emph{symmetrized Hausdorff distance} between two sets $S_0,S_1 \subseteq \R^n$ is defined as the $ \max_{b \in \{0,1\}} \min_{s \in S_b} \max_{t \in S_{1-b}} \frac{\langle s,t \rangle^2}{\|s\|^2\|t\|^2} \geq 1-\epsilon$. We say that two matrices $A, A'$ are $\epsilon$-close in symmetrized Hausdorff distance if the set of columns of $A, A'$ are $\epsilon$-close in symmetrized Hausdorff distance.


% We write $\Perm{[n]}{r}$ for the set of all $r$-tuples formed by taking $r$ \emph{distinct} elements from $[n]$. The Kronecker product $T$ of $v_1 \otimes v_2 \otimes \ldots v_k$ for vectors $v_i \in \R^{n_i}$ is a vector in $\R^{n_1 \times n_2 \times \cdots n_k}$ with entries indexed by tuples $(i_1, i_2, \ldots, i_k)$ where any $i_j \in [n_j]$ defined by $T(i_1, i_2, \ldots, i_k) = \Pi_{j \leq k} v_j(i_j)$. $\|\cdot \|$ for matrices will denote the spectral norm and for vectors, the Euclidean norm.



%Throughout this paper, for a vector $v$, we use $\norm{v}_2$ to denote the Euclidean norm of $v$. 
%For a $n \times m$ matrix $M$, we use $\norm{M}_2 = \max_{\norm{x}_2=1} \norm{Mx}_2$ to denote the spectral norm of $M$ and $\norm{M}_F = \sqrt{\sum_{i,j} M_{i,j}^2}$ to denote the Frobenius norm of $M$. 

% Throughout this paper, for a vector $v$, we use $\norm{v}_2$ to denote the Euclidean norm of $v$. For a $n \times m$ matrix $M$, we use $\norm{M}_2 = \max_{\norm{x}_2=1} \norm{Mx}_2$ to denote the spectral norm of $M$ and $\norm{M}_F = \sqrt{\sum_{i,j} M_{i,j}^2}$ to denote the Frobenius norm of $M$. For symmetric matrices we use $\succeq$ to denote the PSD/Löwner ordering over eigenvalues of $M$. For a $n \times n$, rank-$r$ symmetric matrix $M$, we use $U\Lambda U^{\top}$ to denote the Eigenvalue Decomposition, where $U$ is a $n \times r$ matrix with orthonormal columns and $\Lambda$ is a $r \times r$ diagonal matrix denoting the eigenvalues. We use $M^{\dagger} = U \Lambda^{\dagger} U^{\top} $ to denote the Moore-Penrose pseudoinverse, where $\Lambda^{\dagger}$ inverts the non-zero eigenvalues of $M$. If $M \succeq 0$, we use $M^{\dagger/2} = U \Lambda^{\dagger/2} U^{\top}$ to denote taking the square-root of the non-zero eigenvalues. We use $\Pi = U U^{\top}$ to denote the Projection matrix corresponding to the column/row span of $M$. Since $\Pi = \Pi^2$, the pseudo-inverse of $\Pi$ is itself, i.e. $\Pi^{\dagger} = \Pi$. 


% \begin{definition}[$\sigma$-Sub-gaussian Distribution]
% A random variable $x$ is drawn from a $\sigma$-Sub-gaussian distribution if for all $t\geq0$, 
% $\Pr\left[|x| \geq t \right] \leq 2\exp(-t^2/\sigma^2)$.
% \end{definition}

% We work with $1$-Sub-gaussian distributions unless otherwise specified and drop the $1$ when clear from context. 

% \paragraph{Probability Preliminaries.} We begin with standard convergence results for mean and covariance.

% \begin{fact}[Empirical Mean for Sub-gaussians]
% \label{fact:empirical_mean}
% Let $\cD$ be a Sub-gaussian distribution on $\R^d$ with mean $\mu$ and covariance $\Sigma$ and let $x_1, x_2, \ldots x_n \sim \cD$. Then, with probability $1-\delta$,
% \[
% \Norm{ \frac{1}{n}\sum^n_{i=1} x_i - \mu }_2 \leq \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{\frac{\|\Sigma\|_2 \log(1/\delta)}{n}}
% \]
% \end{fact}



% \begin{fact}[Empirical Covariance for Sub-gaussians, Proposition 2.1 \cite{MR2956207-Vershynin12}]
% \label{fact:empirical_cov}
% Let $\cD$ be a Sub-gaussian distribution on $\mathbb{R}^d$ with mean $\mu$ and covariance $\Sigma$ and let $x_1, x_2, \ldots x_n \sim \cD$. Then, with probability $1-\delta$,
% \[
% \Norm{ \frac{1}{n}\sum^n_{i=1} x_i x_i^{\top} - \Sigma }_2 \leq c \left(\sqrt{\frac{d}{n}} + \sqrt{ \frac{\log(1/\delta)}{n}}\right)
% \]
% \end{fact}

% \begin{definition}[Hellinger Distance]
% For probability distribution $p,q$ on  $\R^d$, let 
% \[
% h(P,Q) = \frac{1}{\sqrt{2}} \sqrt{ \int_{\R^d} \left(\sqrt{p(x)} - \sqrt{q(x)}\right)^2 dx}
% \] 
% be the Hellinger distance between them. 
% \end{definition}

% \begin{remark}
% Hellinger distance between $p,q$ satisfies: $h(p,q)^2 \leq \dtv(p,q) \leq h(p,q)\sqrt{2 -h(p,q)^2}$.  
% \end{remark}

% \begin{fact}[Hellinger Distance between Gaussians] \label{fact:hellinger-gaussians}
% \begin{equation*}
% h(\cN(\mu,\Sigma), \cN(\mu',\Sigma'))^2 =1 - \frac{\det(\Sigma)^{1/4} \det(\Sigma')^{1/4}}{\det\left( \frac{\Sigma+\Sigma'}{2}\right)^{\frac{1}{2}}} \exp\left(-\frac{1}{8} (\mu - \mu)^{\top}\Paren{\frac{\Sigma + \Sigma'}{2}}^{-1} (\mu - \mu') \right)
% \end{equation*}
% \end{fact}


We refer the reader to the monograph~\cite{TCS-086} and the lecture notes~\cite{BarakS16} for a detailed exposition 
of the sum-of-squares method and its usage in average-case algorithm design. 


Let $x = (x_1, x_2, \ldots, x_n)$ be a tuple of $n$ indeterminates and let $\R[x]$ be the set of polynomials 
with real coefficients and indeterminates $x_1,\ldots,x_n$. We say that a polynomial $p\in \R[x]$ is a 
\emph{sum-of-squares (sos)} if there exist polynomials $q_1,\ldots,q_r$ such that $p=q_1^2 + \cdots + q_r^2$.

\subsubsection{Pseudo-distributions}

Pseudo-distributions are generalizations of probability distributions.
We can represent a discrete (i.e., finitely supported) probability distribution over $\R^n$ 
by its probability mass function $D\from \R^n \to \R$ such that $D \geq 0$ 
and $\sum_{x \in \mathrm{supp}(D)} D(x) = 1$.
Similarly, we can describe a pseudo-distribution by its mass function 
by relaxing the constraint $D\ge 0$ to passing certain low-degree non-negativity tests.

Concretely, a \emph{level-$\ell$ pseudo-distribution} is a finitely-supported function $D:\R^n \rightarrow \R$ 
such that $\sum_{x} D(x) = 1$ and $\sum_{x} D(x) f(x)^2 \geq 0$ for every polynomial $f$ of degree at most $\ell/2$.
(Here, the summations are over the support of $D$.)
A straightforward polynomial-interpolation argument shows that every level-$\infty$-pseudo distribution 
satisfies $D\ge 0$ and is thus an actual probability distribution.
We define the \emph{pseudo-expectation} of a function $f$ on $\R^n$ with respect to a pseudo-distribution $D$, 
denoted $\pE_{D(x)} f(x)$, as
\begin{equation}
  \pE_{D(x)} f(x) = \sum_{x} D(x) f(x) \,\mper
\end{equation}
The degree-$\ell$ moment tensor of a pseudo-distribution $D$ is the tensor $\pE_{D(x)} (1,x_1, x_2,\ldots, x_n)^{\otimes \ell}$.
In particular, the moment tensor has an entry corresponding to the pseudo-expectation of all monomials of degree at most $\ell$ in $x$.
The set of all degree-$\ell$ moment tensors of probability distribution is a convex set.
Similarly, the set of all degree-$\ell$ moment tensors of degree-$d$ pseudo-distributions is also convex.
Unlike moments of distributions, there is an efficient separation oracle for moment tensors of pseudo-distributions.
\begin{fact}[\cite{MR939596-Shor87,MR1748764-Nesterov00,MR1846160-Lasserre01,MR3050242-Parrilo13}] 
\label[fact]{fact:sos-separation-efficient}
For any $n,\ell \in \N$, the following set has an $n^{O(\ell)}$-time weak separation oracle 
(in the sense of \cite{MR625550-Grotschel81}):
\begin{equation}
\Set{ \pE_{D(x)} (1,x_1, x_2, \ldots, x_n)^{\otimes d} \mid \text{ degree-d pseudo-distribution $D$ over $\R^n$}}\,\mper
\end{equation}
\end{fact}
This fact, together with the equivalence of weak separation and optimization \cite{MR625550-Grotschel81}, 
allows us to efficiently optimize over pseudo-distributions (approximately) --- this algorithm is referred to as 
the sum-of-squares algorithm. The \emph{level-$\ell$ sum-of-squares algorithm} optimizes over the space 
of all level-$\ell$ pseudo-distributions that satisfy a given set of polynomial constraints (defined below).

\begin{definition}[Constrained pseudo-distributions]
Let $D$ be a level-$\ell$ pseudo-distribution over $\R^n$.
Let $\cA = \{f_1\ge 0, f_2\ge 0, \ldots, f_m\ge 0\}$ be a system of $m$ polynomial inequality constraints.
We say that \emph{$D$ satisfies the system of constraints $\cA$ at degree $r$}, denoted $D \sdtstile{r}{} \cA$, 
if for every $S\subseteq[m]$ and every sum-of-squares polynomial $h$ with 
$\deg h + \sum_{i\in S} \max\set{\deg f_i,r}$, we have that $\pE_{D} h \cdot \prod _{i\in S}f_i  \ge 0$.

We write $D \sdtstile{}{} \cA$ (without specifying the degree) if $D \sdtstile{0}{} \cA$ holds.
Furthermore, we say that $D\sdtstile{r}{}\cA$ holds \emph{approximately} if the above inequalities 
are satisfied up to an error of $2^{-n^\ell}\cdot \norm{h}\cdot\prod_{i\in S}\norm{f_i}$, 
where $\norm{\cdot}$ denotes the Euclidean norm\footnote{The choice of norm is not important here because 
the factor $2^{-n^\ell}$ swamps the effects of choosing another norm.} 
of the coefficients of a polynomial in the monomial basis.
\end{definition}

We remark that if $D$ is an actual (discrete) probability distribution, then we have that 
$D\sdtstile{}{}\cA$ if and only if $D$ is supported on solutions to the constraints $\cA$. 
We say that a system $\cA$ of polynomial constraints is \emph{explicitly bounded} 
if it contains a constraint of the form $\{ \|x\|^2 \leq M\}$.
The following fact is a consequence of \cref{fact:sos-separation-efficient} and \cite{MR625550-Grotschel81}:
\begin{fact}[Efficient Optimization over Pseudo-distributions]
There exists an $(n+ m)^{O(\ell)} $-time algorithm that, given any explicitly bounded and satisfiable 
system\footnote{Here, we assume that the bit complexity of the constraints in $\cA$ is $(n+m)^{O(1)}$.} 
$\cA$ of $m$ polynomial constraints in $n$ variables, outputs a level-$\ell$ pseudo-distribution 
that satisfies $\cA$ approximately. \label{fact:eff-pseudo-distribution}
\end{fact}

\paragraph{Basic Facts about Pseudo-Distributions.}

We will use the following Cauchy-Schwarz inequality for pseudo-distributions:
\begin{fact}[Cauchy-Schwarz for Pseudo-distributions] \label{fact:pseudo-expectation-cauchy-schwarz}
Let $f, g$ be polynomials of degree at most $d$ in indeterminate $x \in \R^d$. 
Then, for any degree-$d$ pseudo-distribution $\tzeta$, we have that
$\pE_{\tzeta}[fg] \leq \sqrt{\pE_{\tzeta}[f^2]} \sqrt{\pE_{\tzeta}[g^2]}$.
\end{fact}

\begin{fact}[H{\"o}lder's Inequality for Pseudo-Distributions] \label{fact:pseudo-expectation-holder}
Let $f, g$ be polynomials of degree at most $d$ in indeterminate $x \in \R^d$. 
Fix $t \in \N$. Then, for any degree-$d t$ pseudo-distribution $\tzeta$, we have that
$\pE_{\tzeta}[f^{t-1}g] \leq \paren{\pE_{\tzeta}[f^t]}^{\frac{t-1}{t}} \paren{\pE_{\tzeta}[g^t]}^{1/t}$.
\end{fact}

\begin{corollary}[Comparison of Norms] \label{fact:comparison-of-pseudo-expectation-norms}
Let $\tzeta$ be a degree-$t^2$ pseudo-distribution over a scalar indeterminate $x$. 
Then, we have that $\pE[x^{t}]^{1/t} \geq \pE[x^{t'}]^{1/t'}$ for every $t' \leq t$. 
\end{corollary}

% \paragraph{Reweighting Pseudo-Distributions}

% The following fact is easy to verify and has been used in several works (see~\cite{DBLP:conf/stoc/BarakKS17} for example).  
% \begin{fact}[Reweightings] \label{fact:reweightings}
% Let $\tmu$ be a pseudo-distribution of degree $k$ satisfying a set of polynomial constraints $\cA$ in variable $x$. 
% Let $p$ be a sum-of-squares polynomial of degree $t$ such that $\pE[p(x)] \neq 0$.
% Let $\tmu'$ be the pseudo-distribution defined so that for any polynomial $f$, $\pE_{\tmu'}[f(x)] = \pE_{\tmu}[ f(x)p(x)]/\pE_{\tmu}[p(x)]$. Then, $\tmu'$ is a pseudo-distribution of degree $k-t$ satisfying $\cA$. 
% \end{fact}

\subsubsection{Sum-of-squares proofs}

Let $f_1, f_2, \ldots, f_r$ and $g$ be multivariate polynomials in $x$.
A \emph{sum-of-squares proof} that the constraints $\{f_1 \geq 0, \ldots, f_m \geq 0\}$ imply the constraint $\{g \geq 0\}$ 
consists of  polynomials $(p_S)_{S \subseteq [m]}$ such that
\begin{equation}
g = \sum_{S \subseteq [m]} p_S \cdot \Pi_{i \in S} f_i \mper
\end{equation}
We say that this proof has \emph{degree $\ell$} if for every set $S \subseteq [m]$ 
the polynomial $p_S \Pi_{i \in S} f_i$ has degree at most $\ell$.
If there is a degree $\ell$ SoS proof that $\{f_i \geq 0 \mid i \leq r\}$ implies $\{g \geq 0\}$, we write:
\begin{equation}
\{f_i \geq 0 \mid i \leq r\} \sststile{\ell}{}\{g \geq 0\} \mper
\end{equation}
For all polynomials $f, g\colon \R^n \to \R$ and for all functions $F\colon \R^n \to \R^m$, 
$G\colon \R^n \to \R^k$, $H\colon \R^{p} \to \R^n$ such that each of the coordinates of the outputs are polynomials of the inputs, 
we have the following inference rules.

The first one derives new inequalities by addition or multiplication:
\begin{equation} \label{eq:sos-addition-multiplication-rule}
\frac{\cA \sststile{\ell}{} \{f \geq 0, g \geq 0 \} } {\cA \sststile{\ell}{} \{f + g \geq 0\}}, \frac{\cA \sststile{\ell}{} \{f \geq 0\}, \cA \sststile{\ell'}{} \{g \geq 0\}} {\cA \sststile{\ell+\ell'}{} \{f \cdot g \geq 0\}}\mper
\end{equation}
The next one derives new inequalities by transitivity: 
\begin{equation} \label{eq:sos-transitivity}
\frac{\cA \sststile{\ell}{} \cB, \cB \sststile{\ell'}{} C}{\cA \sststile{\ell \cdot \ell'}{} C}\mper 
\end{equation}
Finally, the last rule derives new inequalities via substitution:
\begin{equation} \label{eq:sos-substitution}
\frac{\{F \geq 0\} \sststile{\ell}{} \{G \geq 0\}}{\{F(H) \geq 0\} \sststile{\ell \cdot \deg(H)} {} \{G(H) \geq 0\}}\tag{substitution}\mper
\end{equation}
Low-degree sum-of-squares proofs are sound and complete if we take low-level pseudo-distributions as models.
Concretely, sum-of-squares proofs allow us to deduce properties of pseudo-distributions that satisfy some constraints.
\begin{fact}[Soundness] \label{fact:sos-soundness}
If $D \sdtstile{r}{} \cA$ for a level-$\ell$ pseudo-distribution $D$ and there exists a sum-of-squares proof 
$\cA \sststile{r'}{} \cB$, then $D \sdtstile{r\cdot r'+r'}{} \cB$.
\end{fact}
If the pseudo-distribution $D$ satisfies $\cA$ only approximately, soundness continues to hold 
if we require an upper bound on the bit-complexity of the sum-of-squares $\cA \sststile{r'}{} B$ 
(i.e., the number of bits required to write down the proof). In our applications, the bit complexity of all 
sum-of-squares proofs will be $n^{O(\ell)}$ (assuming that all numbers in the input have bit complexity $n^{O(1)}$). 
This bound suffices in order to argue about pseudo-distributions that satisfy polynomial constraints approximately.

The following fact shows that every property of low-level pseudo-distributions can be derived by low-degree sum-of-squares proofs.
\begin{fact}[Completeness] \label{fact:sos-completeness}
Suppose that $d \geq r' \geq r$ and $\cA$ is a collection of polynomial constraints with degree at most $r$, 
and $\cA \sststile{}{} \{ \sum_{i = 1}^n x_i^2 \leq B\}$ for some finite $B$.
Let $\{g \geq 0 \}$ be a polynomial constraint. If every degree-$d$ pseudo-distribution that satisfies $D \sdtstile{r}{} \cA$ 
also satisfies $D \sdtstile{r'}{} \{g \geq 0 \}$, then for every $\epsilon > 0$, 
there is a sum-of-squares proof $\cA \sststile{d}{} \{g \geq - \epsilon \}$.
\end{fact}

\paragraph{Basic Sum-of-Squares Proofs.}
We will require the following basic SoS proofs.

\begin{fact}[Operator norm Bound] \label{fact:operator_norm}
Let $A$ be a symmetric $d\times d$ matrix and $v$ be a vector in $\mathbb{R}^d$. Then, we have that
\[\sststile{2}{v} \Set{ v^{\top} A v \leq \|A\|_2\|v\|^2_2 } \;.\]
\end{fact}

\begin{fact}[SoS H{\"o}lder's Inequality] \label{fact:sos-holder}
Let $f_i, g_i$, for $1 \leq i \leq s$, be scalar-valued indeterminates. 
Let $p$ be an even positive integer.  
Then, 
\[
\sststile{p^2}{f,g} \Set{  \Paren{\frac{1}{s} \sum_{i = 1}^s f_i g_i^{p-1}}^{p} \leq \Paren{\frac{1}{s} \sum_{i = 1}^s f_i^p} \Paren{\frac{1}{s} \sum_{i = 1}^s g_i^p}^{p-1}}\mper
\]
\end{fact}
\noindent Observe that using $p =2$ above yields the SoS Cauchy-Schwarz inequality. 

\begin{fact}[SoS Almost Triangle Inequality] \label{fact:almost-triangle-sos}
Let $f_1, f_2, \ldots, f_r$ be indeterminates. Then, we have that
\[
\sststile{2t}{f_1, f_2,\ldots,f_r} \Set{ \Paren{\sum_{i\leq r} f_i}^{2t} \leq r^{2t-1} \Paren{\sum_{i =1}^r f_i^{2t}}}\mper
\]
\end{fact}


\begin{fact}[SoS AM-GM Inequality, see Appendix A of~\cite{MR3388192-Barak15}] \label{fact:sos-am-gm}
Let $f_1, f_2,\ldots, f_m$ be indeterminates. Then, we have that
\[
\sststile{m}{f_1, f_2,\ldots, f_m} \Set{ \Paren{\frac{1}{m} \sum_{i =1}^n f_i }^m \geq \Pi_{i \leq m} f_i} \mper
\]
\end{fact}

We defer the proofs of the two subsequent lemmas to Appendix \ref{sec:omitted_proofs}.

\begin{lemma}[Spectral SoS Proofs] \label{lem:spectral-sos-proofs}
Let $A$ be a $d \times d$ matrix. Then for $d$-dimensional vector-valued indeterminate $v$, we have:
\[
\sststile{2}{v} \Set{ v^{\top}Av \leq \Norm{A}_2 \Norm{v}_2^2}\mper
\]
\end{lemma}

\begin{fact}[Cancellation within SoS, Lemma 9.2~\cite{BK20}]
Let $a,C$ be scalar-valued indeterminates. Then, 
\[
\Set{a \geq 0} \cup \Set{a^t \leq C a^{t-1}} \sststile{2t}{a,C} \Set{a^{2t} \leq C^{2t}}\mper
\]
\label{fact:sos-cancellation}
\end{fact}



\begin{lemma}[Frobenius Norms of Products of Matrices] \label{lem:frob-of-product}
Let $B$ be a $d \times d$ matrix valued indeterminate for some $d \in \N$. Then, for any $0 \preceq A \preceq I$, 
\[
\sststile{2}{B} \Set{\Norm{AB}_F^2 \leq \Norm{B}_F^2}\mcom
\]
and, 
\[
\sststile{2}{B} \Set{\Norm{BA}_F^2 \leq \Norm{B}_F^2}\mcom
\]
\end{lemma}

% The following fact is a simple corollary of the fundamental theorem of algebra:

% \begin{fact}
% For any univariate degree $d$ polynomial $p(x) \geq 0$ for all $x \in \R$,
% $\sststile{d}{x} \Set{p(x) \geq 0}$.
%  \label{fact:univariate}
% \end{fact}

% This can be extended to univariate polynomial inequalities over intervals of $\R$.
% 2\begin{fact}[Fekete and Markov-Lukacs, see \cite{laurent2009sums}]
% For any univariate degree $d$ polynomial $p(x) \geq 0$ for $x \in [a, b]$,  $\Set{x\geq a, x \leq b} \sststile{d}{x} \Set{p(x) \geq 0}$.  \label{fact:univariate-interval}
% \end{fact}



% \subsection{Certifiable Anti-Concentration}
% This definition is a homogenous variant of the one proposed in ~\cite{DBLP:journals/corr/abs-1905-05679}.
% \begin{definition}[Certifiable Anti-Concentration]
% A zero-mean distribution $D$ with covariance $\Sigma$ is $2k$-certifiably $(\delta,C\delta)$-anti-concentrated if there exists a univariate polynomial $p$ of degree $k$ such that:
% \begin{enumerate}
% \item $\sststile{2k}{v} \Set{\norm{v}_2^{2k-2} \iprod{\Sigma^{-1/2} x,v}^2 + \delta^2 p^2\paren{\iprod{\Sigma^{-1/2} x,v}} \geq \delta^2 \norm{v}_2^{2k}}$. 
% \item $\sststile{2k}{v} \Set{\E_{\Sigma^{-1/2} x \sim D} p^2\paren{\iprod{\Sigma^{-1/2} x,v}} \leq C\delta \norm{v}_2^{2k}}$.
% \end{enumerate}
% A subset $X \subseteq  \R^d$ is $2k$-certifiably $(\delta,C\delta)$-anti-concentrated if the uniform distribution on $X$ is $2k$-cerfiably $(\delta,C\delta)$-anti-concentrated.
% \label{def:certifiable-anti-concentration-homogenous}
% \end{definition}
% \FIXME{A: maybe we should define this using pseudo inverses.}
% \begin{definition}[Certifiable Anti-Concentration] \label{def:certified-anti-concentration}
% A random variable (and its distribution) $Y$ has a $k$-\emph{certifiably} $(C,\delta)$-anti-concentrated distribution if there is a univariate polynomial $p$ satisfying $p(0) = 1$ such that there is a degree $k$ sum-of-squares proof of the following two inequalities: 
% \begin{enumerate} 
% \item $\langle Y,v\rangle^2 \leq \delta^2 \E \langle Y,v\rangle^2$ implies $(p(\langle Y,v\rangle) -1)^2\leq \delta^2$.
% \item $\forall v$, $\E \iprod{Y,v}^2 >0$ implies  $\E \left[ \E\iprod{Y,v}^2 p^2(\left \langle Y,v\rangle \right) \right] \leq C\delta \iprod{Y,v}^2$.
% \end{enumerate}
% A set of points $S \subseteq \R^d$ are said to be $k$-certifiably $(C,\delta)$-anti-concentrated if uniform distribution on $S$ is $k$-certifiably $(C,\delta)$-anti-concentrated. 
% \end{definition} 


==> robust_mean_covariance.tex <==
%!TEX root = main.tex


\section{Robustly Estimating Covariance of the Mixture}


We require estimating the mean and covariance of the mixture of $k$ Gaussians. 

\begin{theorem}[Robust Mean and Covariance for a Mixture]
\label{thm:robust_mean_and_covariance_estimation}
Let  $\calG = \sum_{i \in [k]} w_i \calN\Paren{\mu_i, \Sigma_i}$ be a mixture of $k$ Gaussians and let $\mu = \sum_{i \in [k]} w_i \mu_i $, $\Sigma = \sum_{i \in [k]} w_i \Sigma_i$ be the mean and covariance of $\calG$. Given $n \geq n_0$ $\epsilon$-corrupted samples from $\calG$, there exists an algorithm that runs in time $\poly(n)$ and outputs estimators $\hat{\mu}$ and $\hat{\Sigma}$ such that when $n_0 = \poly(d\log(d))$, with probability $99/100$,
\begin{enumerate}
  \item Mean Estimation : 
  \[ 
  \Norm{\Sigma^{-1/2} \Paren{\mu - \hat{\mu}} }_2 \leq \bigO{\epsilon^{1/2}/w_{\min} }
  \]
  \item Covariance Estimation :
  \[
  \Norm{\Sigma^{-1/2} \hat{\Sigma} \Sigma^{-1/2}  - \II }_F \leq \bigO{\epsilon /w_{\min}}
  \]
\end{enumerate}
\end{theorem}

We show that the uniform distribution over a sufficiently large set of uncorrupted samples from a mixture of $k$ Gaussians satisfies certifiably hypercontractivity of degree $2$ polynomials. 

\begin{definition}[Certifiable Hypercontractivity]
Let $\cD$ be a distribution on $\R^d$. For an even $k$, $\cD$ is said to have $h$-certifiably $C$-hypercontractive degree $2$ polynomials if for $P$ - a $d \times d$ matrix-valued indeterminate, 
\begin{equation*}
\sststile{2h}{P} \Set{ \E_{x \sim \cD} \iprod{P,x^{\otimes 2}}^h \leq (Ch)^{h} \Norm{P}_2^h } \mper
\end{equation*}
\end{definition}

We use the following result from Kauers, O'Donnell, Tan and Zhou \cite{DBLP:conf/soda/KauersOTZ14}: 

\begin{fact}[Certifiable Hypercontractivity of a Gaussian]
The standard normal distributio, $\calN\Paren{0,\II}$, has $h$-certifiably $1$-hypercontractive degree $2$ polynomials. 
\end{fact}

We are now ready to show the key lemma:

%\anote{there is a slight issue here with comparing the mean of the mixture to the mixture of the components.}

\begin{lemma}[Certifiable Hypercontractivity of a Gaussian Mixture]
A mixture of $k$-Gaussians, denoted by $\calG = \sum_{i \in [k]} w_i \calN\Paren{\mu_i, \Sigma_i}$ has $h$-certifiably $\bigO{1/w_{\min}}$ hypercontractive degree $2$ polynomials. 
\end{lemma}
\begin{proof}
We begin by assuming the mean of the mixture $\calG$ is $0$. \anote{when the mean is non-zero, we first robustly estimate the mean, which only requires certifiable sub-gaussianity and then subtract it off. I'll add this below to the sampling part.}
\begin{equation}
\begin{split}
 \E_{x \sim \calG } \left[ \Iprod{ x , P x}^h \right] & = \sum_{i \in [k]} w_i \E_{x \sim \calN\Paren{\mu_i , \Sigma_i} } \left[ \Iprod{ x , P x}^h \right]  \\
 & = \sum_{i \in [k]} w_i \E_{x \sim \calN\Paren{0 , \II } } \left[ \Iprod{ x-\mu_i , \Sigma_i^{1/2} P \Sigma_i^{1/2} \Paren{ x - \mu_i} }^h \right]\\
 & \leq \Paren{h/w_{\min} }^h \sum_{i \in [k]} \Norm{ w_i   \Sigma_i^{1/2} P \Sigma_i^{1/2}  }^h_F \\
 & = \Paren{h/w_{\min} }^h \sum_{i \in [k]} \Norm{ w_i   \Sigma_i P   }^h_F \\
 & \leq \Paren{h/w_{\min} }^h  \Norm{\sum_{i \in [k]}  w_i    \Sigma_i P   }^h_F \\
 & =   \Paren{h/w_{\min} }^h  \Norm{ \Sigma^{1/2} P \Sigma^{1/2}  }^h_F
\end{split}
\end{equation}
where we repeatedly use that for a PSD matrix $A = A^{1/2}A^{1/2}$ and a symmetrix matrix $P$, $\Norm{A^{1/2} P A^{1/2}}^2_F = \trace{A^{1/2} P A P A^{1/2} } = \trace{A P A P  } = \Norm{A P }^2_F$.
\end{proof}


To conclude, we use the fact that sampling preserves certifiable hypercontractivty of degree $2$ polynomials :

\begin{lemma}[Sampling preserves Certifiable Hypercontractivity, Lemma 8.3 \cite{bakshi2020mixture}]
Let $\calD$ be a $1$-subgaussian distribution with $h$-certifiably $c$-hypercontractive  degree $2$ polynomials over $\R^d$ and let $\calS = \{ x_1 , x_2, \ldots x_n \}$ be $n \geq n_0$ i.i.d. samples from $\calD$. Then, with probability at least $1-1/n$, the uniform distribution over $\calS$ has $h$-certifiably $(2c)$-hypercontractive degree $2$ polynomials, when $n_0 = \bigOmega{ {hd}^{8h} }$.
\end{lemma}

The claim then follows from Theorem 7.1 in \cite{bakshi2020mixture}

==> td_upto_low_rank-old.tex <==
%!TEX root = main.tex

In this section, we prove Proposition~\ref{prop:tensor_decomposition_upto_lowrank}.
We first set some useful notation. We will write $\Sigmaa_i \eqdef \Sigma_i-I$ throughout this section.
We will also use $\Sigmaa_i'$ to denote $\Sigmaa_i + \mu_i \otimes \mu_i$.
% \begin{lemma}[Tensor Decomposition up to Low-Rank Error]
% \label{lem:tensor_decomposition_upto_lowrank}
% Given $0<\eta<1$, let $\hat{T}_4$ be a tensor such that $\Norm{\E[h_4(\calX)]- \hat{T}_4 }_F \leq \eta$, let $D = \bigO{ k^4/(\alpha \sqrt{\eta} }$, $\Delta$ be the upper bound the individual covariances in relative Frobenius norm.
% For all $j \in [t]$, let $x^{(j)}, y^{(j)} \sim \calN(0, I)$ and $a_j \sim \calU[-D, D]$ , and let $\hat{\Sigmaa} = \sum_{j\in[t]} a_j \hat{T}_{4}\Paren{\cdot, \cdot ,x^{(j)},y^{(j)}}$. Then, for each $i \in [k]$, with probability at least $ \Paren{ \eta /\Paren{ k^5\Paren{\Delta^4 + 1/\alpha^4 }} }^{4k} $, over the  choice of $x_j,y_j$ and $a_j$, we have that $\hat{\Sigmaa}-\Sigmaa_i = P_i + Q_i$, where $\Norm{P_i}_F = \bigO{ \sqrt{\eta}}$, $\Norm{Q_i}_F =\bigO{ \frac{1}{\sqrt{\eta}\alpha} \Paren{\Delta^2 + \frac{1}{\alpha^4} } }$
% %$\Norm{P_i}_F = \bigO{\poly(\eta k\log(k)/\alpha \epsilon) +\epsilon}$
% and $\textrm{rank}(Q_i) = \bigO{k^2}$.
% \end{lemma}


% \begin{proposition}
% Let $T$ be a tensor so that $|\E[h_4(X)]-T|_F \leq \eta\leq 1$. Let $\Sigmaa'_{i_1i_2} = \sum_{j=1}^{2k} a_jT_{i_1i_2i_3i_4}x^j_{i_3}y^j_{i_4}$ where the $x^j$ and $y^j$ are independent Gaussian random variables and the $a_j$ are uniform random variables in $[-D,D]$ where $D$ is a sufficiently large multiple of $k^3/(\alpha \eps)$. Then with probability at least $\poly_k(\eps)$ we have that $\Sigmaa'-\Sigmaa_i$ is the sum of a matrix of Frobenius norm $O(\eta\log(k)+\eps)$ plus a matrix of rank $O(k^2)$.
% \end{proposition}


We first show that for every $i$, there exists a matrix $P$ such that $\Paren{\sum_{i\in [k]} w_i \Sigmaa'_i \otimes \Sigmaa'_i } \Paren{\cdot, \cdot, P}$ is close to $\Sigmaa'_i$.

\begin{lemma}[Existence of a $2$-Tensor] \label{lem:existence_2_tensor}
Under the hypothesis of Proposition~\ref{prop:tensor_decomposition_upto_lowrank}, for each $i\in[k]$,
there exists a matrix $P$ such that $\Norm{P}_F =  \bigO{1/(\sqrt{\eta} \alpha)}$ and
$\Norm{ T'_4\Paren{\cdot, \cdot, P} - \Sigmaa_i'}_F = \bigO{\sqrt{\eta/\alpha}}$,
where $T'_4 = \Paren{\sum_{i\in [k]} w_i \Sigmaa'_i \otimes \Sigmaa'_i }$.
\end{lemma}


Before we prove Lemma \ref{lem:existence_2_tensor}, we need the following duality fact:

\begin{fact}[Duality for Closed Convex Sets]
\label{fact:duality_compact}
Given a $m \times n$ matrix $A$, $b \in \R^m$, and a closed convex set $K \in \R^n$,
let $Ax \leq_{K} b$ denote the set of constraints for $Ax \leq b$, for all $x \in K$.
Then, the constraint system $Ax \leq_{K} b$ is satisfiable iff $0 < \gamma$
is not a constraint in $Ax \leq_{K} b$, for all $\gamma <0$.
\end{fact}

\begin{proof}[Proof of Lemma \ref{lem:existence_2_tensor}]
% We claim that with high probability over the choice of $x^j$ and $y^j$ that there exist real numbers $b_j$ with $|b_j|\leq D$ so that $\sum_{j=1}^{2k} b_j (T_4')x^j y^j = \Sigmaa_i'+O(\eps)$. Then so long as $x^j$ and $y^j$ satisfy the above and $a_j$ is close to $b_j$ for all $j$, our result will hold (noting that $\Sigmaa_i$ and $\Sigmaa_i'$ differ by a rank 1 matrix).
% To show that the $b_j$ exist, first we claim that there is a $2$-tensor $P$ so $|P|_2 \leq 1/(\eps\alpha)$ and so that $|(T_4')P - \Sigmaa_i'|_2 = O(\eps)$.

To show that such a $P$ exists for each $i$, we apply linear programming duality.
In particular, the conditions imposed on $P$ define a linear program, which has a feasible
solution unless there is a solution to the dual linear program.
Consider the following primal in the variable $P$:
\begin{align} \label{eqn:primal}
\Iprod{v, P}  & \leq \frac{c_1}{ \sqrt{\eta} \alpha} \Norm{v}_F     &  \forall\hspace{0.1in} v \in \mathbb{R}^{d \times d} \\
\label{eqn:primal_a}
\Iprod{u, T'_4\Paren{\cdot, \cdot, P} - \Sigmaa'_i } & \leq c_2\sqrt{\eta}  \Norm{u}_F
& \forall\hspace{0.1in} u \in \mathbb{R}^{d \times d}
\end{align}
for sufficiently large constants $c_1$ and $c_2$.
Throughout the proof, we suggest that the reader considers $v, u$ to be vectors in $d^2$-dimensional vector space.


% If the LP is infeasible, by Farkas' lemma, there exist $y_i\ge0$ and $z_j\ge0$ and $v_i,u_j\in\R^{d\times d}$ such that
% $$
% \begin{cases}
% \sum_i y_i v_i+\sum_j z_jT'_4(u_j,\cdot,\cdot)=0\\
% \sum_i y_i\frac{\norm{v_i}_F}{\sqrt{\eta}\alpha}+\sum_j z_j\left(\norm{u_j}_FO(\sqrt{\eta})-\langle u_j,\Sigmaa'_i\rangle\right)<0.
% \end{cases}
% $$
% Let $v=\sum_i y_i v_i$ and $T'_4(u,\cdot,\cdot)=\sum_j z_j T'_4(u_j,\cdot,\cdot)$.
% Then we have $v+T'_4(u,\cdot,\cdot)=0$ and by triangle inequality,
% $$\frac{\norm{v}_F}{\sqrt{\eta}\alpha}+\norm{u}_FO(\sqrt{\eta})-\langle u,\Sigmaa'_i\rangle\le\sum_i y_i\frac{\norm{v_i}_F}{\sqrt{\eta}\alpha}+\sum_j z_j\left(\norm{u_j}_FO(\sqrt{\eta})-\langle u_j,\Sigmaa'_i\rangle\right) <0.$$
% Then
% \begin{equation}\label{eqn:lower-bound}
% \langle u,\Sigmaa'_i\rangle>\frac{\norm{T'_4(u,\cdot,\cdot)}_F}{\sqrt{\eta}\alpha}+\norm{u}_FO(\sqrt{\eta}).
% \end{equation}
% Given the definition of $T'_4$: $T'_4=\sum_{i=1}^kw_i(\Sigmaa'_i\otimes \Sigmaa'_i)$, we have that $T'_4(u,u)\ge w_i\langle u,\Sigmaa'_i\rangle^2$. Therefore, for any matrix $u$ we have that
% \begin{equation}\label{eqn:upper-bound}
% \norm{u}_F\norm{T'_4(u,\cdot,\cdot)}_F\ge\alpha\langle u,\Sigmaa'_i\rangle^2.
% \end{equation}
% By the AM-GM inequality, we have that
% $$
% \left(\frac{\norm{T'_4(u,\cdot,\cdot)}_F}{\sqrt{\eta}\alpha}+\norm{u}_FO(\sqrt{\eta})\right)^2
% \ge \frac{4}{\alpha}\norm{u}_F\norm{T'_4(u,\cdot,\cdot)}_F \;.
% $$
% Then (\ref{eqn:lower-bound}) and (\ref{eqn:upper-bound}) contradict each other.

%\Anote{editing here. Using a compactness based duality agument  we can switch the order of quantifiers. }

Our goal is to show that there exists a feasible solution $P$ such that \eqref{eqn:primal} and \eqref{eqn:primal_a} hold simultaneously for all $u, v \in \R^{d\times d}$.
Using LP duality over closed and compact convex sets (Fact~\ref{fact:duality_compact}),
it suffices to show that, for all $u, v\in \R^{d\times d}$, there exists a $P$ such that:
\begin{align}
\label{eqn:dual}
\Iprod{v, P} + \Iprod{u, T'_4\Paren{\cdot, \cdot, P} }  -\Iprod{u, \Sigmaa'_i }  & \leq \frac{c_1}{\sqrt{\eta} \alpha} \Norm{v}_F   +  c_2 \sqrt{\eta}  \Norm{u}_F + \zeta \;,
\end{align}
for some fixed small universal constant $0<\zeta<1$. Note that we need to introduce the shift $\zeta$
to satisfy the compactness assumption in Fact \ref{fact:duality_compact}. Observe that
this suffices to obtain the bounds on $P$ and $T'(\cdot, \cdot, P)-S'_i$ by scaling up $u, v$ such that
$\zeta \leq \frac{c_1}{\sqrt{\eta}\alpha} \Norm{v}_F$ and $\zeta \leq c_2 \sqrt{\eta}\Norm{u}_F$.
In the remainder of the argument, we assume that $\Norm{v}_F \geq 1$ and $\Norm{u}_F\geq$1,
and thus drop the $\zeta$.

%The forward direction follows from taking a linear combination of \eqref{eqn:primal} and \eqref{eqn:primal_a}. For the reverse direction, we know Equation \eqref{eqn:dual} is feasible for all $u,v$. Then, setting $u = 0$ and $v=0$ independently yields feasibility of \eqref{eqn:primal}  and \eqref{eqn:primal_a} respectively.
%observe if for any $u, v$, $\Iprod{v, P} + \Iprod{u, T'_4\Paren{\cdot, \cdot, P} }  -\Iprod{u, \Sigmaa'_i }  > \frac{c_1}{\sqrt{\eta} \alpha} \Norm{v}_F   +  c_2 \sqrt{\eta}  \Norm{u}_F$, then $\Iprod{v, P}   \leq \frac{c_1}{ \sqrt{\eta} \alpha} \Norm{v}_F $ and $\Iprod{u, T'_4\Paren{\cdot, \cdot, P} - \Sigmaa'_i } \leq c_2\sqrt{\eta}  \Norm{u}_F$ cannot simultaneously be true.


To simplify Equation \eqref{eqn:dual}, we set $v = - T'_4\Paren{u, \cdot, \cdot} $, and since $\Iprod{u, T'_4\Paren{\cdot, \cdot, P} } = \Iprod{T'_4\Paren{u, \cdot, \cdot} , P }$, we have that for all $u$, there exists a $P$ such that:
\begin{align}
\label{eqn:dual2}
\Iprod{ -T'_4\Paren{u, \cdot, \cdot} + T'_4\Paren{u, \cdot, \cdot}, P}   -\Iprod{u, \Sigmaa'_i }  & \leq \frac{c_1}{\sqrt{\eta} \alpha} \Norm{T'_4\Paren{u, \cdot, \cdot}}_F   +  c_2 \sqrt{\eta}  \Norm{u}_F \;.
\end{align}
%\forall\hspace{0.1in} u \in \mathbb{R}^{d \times d}
Assume, for sake of contradiction, that there exists a $u$ such that
\eqref{eqn:dual2} is false for any setting of $P$. Note, since we set $v$ such that the coefficient of $P$ in Equation \eqref{eqn:dual2} is $0$, it suffices to show that any such $u$ yields a contradiction.
Then, squaring both sides, we have:
%To obtain a contradiction we need to be orthogonal to $P$, and since $\Iprod{u, \hat{T}_4\Paren{\cdot, \cdot, P} } = \Iprod{T'_4\Paren{u, \cdot, \cdot} , P }$, it suffices to set $v = - T'_4\Paren{u, \cdot, \cdot} $. Then, by assumption, there exists a $u$ such that
\begin{equation}
\label{eqn:contradict_this}
\begin{split}
\Iprod{u, \Sigmaa'_i}^2 & >  \Paren{ \frac{c_1}{ \sqrt{\eta} \alpha} \Norm{ T'_4\Paren{u, \cdot, \cdot} }_F  +  c_2 \sqrt{\eta} \Norm{u}_F  }^2\\
& \geq \frac{c}{ \alpha}  \Norm{ T'_4\Paren{u, \cdot, \cdot} }_F \cdot \Norm{u}_F \;,
\end{split}
\end{equation}
for some large enough constant $c>1$, where the last inequality follows from the AM-GM inequality.
However, using the dual characterization of the Frobenius norm, we have
\begin{equation}
\label{eqn:dual_frob}
\begin{split}
\Norm{ T'_4\Paren{u, \cdot, \cdot} }_F & \geq  \frac{\Iprod{ u , T'_4\Paren{u, \cdot, \cdot} } }{\Norm{u}_F}
\geq \frac{w_i}{\Norm{u}_F} \Iprod{ u , \Sigmaa'_i}^2 \;,
\end{split}
\end{equation}
where the last inequality follows from $T'_4$ containing a $w_i \Sigmaa_i\otimes \Sigmaa_i$ term.
Rearranging Equation~\eqref{eqn:dual_frob}, we have
\begin{equation*}
 \Iprod{ u , \Sigmaa'_i}^2  \leq  \frac{ 1}{ w_i } \Norm{ T'_4\Paren{u, \cdot, \cdot} }_F \Norm{u}_F + \frac{\eta}{w_i} \Norm{u}^2_F \leq \frac{1}{\alpha}\Norm{ T'_4\Paren{u, \cdot, \cdot} }_F \Norm{u}_F +  \frac{\eta}{\alpha} \Norm{u}^2_F \;.
\end{equation*}
This contradics Equation~\eqref{eqn:contradict_this}
 and suffices to show feasibility of the primal.
\end{proof}

% Setting this up more formally, the LP in question states that for any $2$-tensors $v$ and $u$ that $v\cdot P \leq |v|_2/(\eps\alpha)$ and $(u T_4')\cdot P-u\cdot \Sigmaa_i' = O(\eps)|u|_2$. For a contradiction to be reached, we must have $v=u T_4'$ and $|u\cdot \Sigmaa_i'| > O(\eps)|u|_2+|v|_2/(\eps\alpha) = O(\eps)|u|_2+|T_4' u|_2/(\eps\alpha)$. However, given the definition of $T_4'$, we have that $u\cdot (T_4' u) \geq w_i |u \cdot \Sigmaa_i'|^2$. Therefore, for any $u$ we have that
% $$
% |T_4' u|_2 \geq \alpha|u\cdot \Sigma_i'| \left(\frac{|u\cdot \Sigma_i'|}{|u|_2}\right).
% $$
% Now if $|u\cdot \Sigmaa_i'| \leq \eps|u|_2$, we are already done. But otherwise $|T_4' u| \geq \eps\alpha |u\cdot \Sigmaa_i'|$ which is sufficient.



We now show that, with high probability, any matrix $P$ obtained in the above lemma
can be approximated by a linear combination of random bi-linear forms,
restricted to the $k$-dimensional subspace of $\mathbb{R}^{d}\times \mathbb{R}^{d}$
spanned by  $\Sigmaa'_i$, for all $i \in [k]$.
%This is sufficient since $T'_4 = \sum_{i \in [k]} w_i S'_i \otimes S'_i$ depends only on the span

\begin{lemma}[Existence of a Bi-Linear Form] \label{lem:existence_of_bilinear}
Given the preconditions in Proposition \ref{prop:tensor_decomposition_upto_lowrank},
with probability at least $1-1/{\poly(k)}$ over the choice of $x^{(j)},y^{(j)}$,
there exist $b_j \in [-D, D]$ for $j \in [4k]$, where $D = \bigO{k^4/(\sqrt{\eta}\alpha)}$,
such that the projection of $\sum_{j=1}^{t} b_j x^{(j)}\otimes y^{(j)}$ onto the space spanned
by the $\Sigmaa_i'$ is $P$, where $P$ satisfies the conclusion of Proposition \ref{lem:existence_2_tensor}.
%We note that this will imply that $(T_4')\left(\sum_{i=1}^{2j} b_j x^j\otimes y^j \right) = (T_4')P$, which is sufficient.
\end{lemma}
\begin{proof}
To prove this lemma, we again use a linear programming based argument.
Consider the following (primal) linear program in the variables $b_j$, for $j \in [4k]$:
\begin{align}\label{eqn:primal_2}
\sum_{j \in [4k]} b_j \langle v, x^{(j)} \otimes y^{(j)} \rangle
& = \langle v,P \rangle   & \forall\hspace{0.1in} v \in \textrm{span}\{\Sigmaa'_i\}  \\
\label{eqn:primal_2_a}
-D  \leq b_j &\leq D   & \forall\hspace{0.1in} j \in [4k]
\end{align}
We want to show that there exists a valid assignment to $b_j$, for $j \in[4k]$,
such that $\abs{b_j} \leq D$ and \eqref{eqn:primal_2} holds for all $v\in \textrm{span}\{\Sigmaa'_i\}$.
We again use Fact \ref{fact:duality_compact} and show that for any $v$ in the span of the $\Sigmaa'_i$s,
there exists an assignment to the $b_j$'s such that
%Taking a linear combination of the constraints we have,
\begin{align} \label{eqn:dual_bilinear}
\Iprod{ v, \sum_{j \in [4k]} b_j  \Paren{x^{(j)} \otimes y^{(j)} }  } +  \sum_{j \in [4k]} u_j \Paren{ \abs{b_j}-D } & \leq \Iprod{v, P} + \zeta \;,
\end{align}
for a fixed universal constant $0< \zeta<1$. We can again consider $\Norm{v}_F \geq 1$
by concluding $\abs{b_j} \leq D +\zeta$, and increasing the bound on $D$ by a constant.
%Assume for sake of contradiction, there exist a $v$ and $u$ that make \eqref{eqn:dual_2} infeasible.
%Recall, Equations \eqref{eqn:primal_2} and \eqref{eqn:primal_2_a} are simulatenously feasible if and only if \eqref{eqn:dual_bilinear} is feasible.
We then simplify \eqref{eqn:primal_2} and remove the dependence on $u$ by setting $b_j$ to be $-\textrm{sign}\Paren{ \Iprod{v, \Paren{x^{(j)} \otimes y^{(j)} } } } \cdot D$, which is a valid assigment. Then, we have
\begin{align}
\label{eqn:dual_bilinear2}
\sum_{j \in [4k]} -D \cdot\abs{\Iprod{ v,  b_j  \Paren{x^{(j)} \otimes y^{(j)} }  } }  & \leq \Iprod{v, P}                        &  \forall\hspace{0.1in} v \in \textrm{span}\{\Sigmaa'_i\}
\end{align}
Then, to show the feasibility of Equation \eqref{eqn:primal_2}, it suffices to show the feasibility of \eqref{eqn:dual_bilinear2}. Assume for sake of contradiction that there exists a $v \in \textrm{span}\{\Sigmaa'_i\} $ such that \eqref{eqn:dual_bilinear2} is false.

% Thus,
% \begin{equation}
% \label{eqn:contradict_using_anticonc}
% 0  > \Iprod{v, P} + \underbrace{\sum_{j \in [t]} D \abs{ \Iprod{ v,  QQ^{\top} \Paren{x^{(j)} \otimes y^{(j)} }  } } }_{(i)}
% \end{equation}

% We will prove the feasibility by contradiction.
% If the LP is infeasible, by Farkas' lemma, there exist $y_i$ and $z_j^{+},z_j^{-}\ge0,j\in[4k]$ and $v_i\in \mathrm{span}\{\Sigmaa'_i\}$
% such that
% $$
% \begin{cases}
% \sum_i y_i \langle v_i,x^{(j)} \otimes y^{(j)}\rangle+z_j^{-}-z_j^{+}=0& \forall j\in[4k]\\
% \sum_i y_i\langle v_i,P\rangle+ D\sum_j(z_j^++z_j^-)<0 \;.
% \end{cases}
% $$
% Let $v=\sum_i y_i v_i\in \mathrm{span}\{\Sigmaa'_i\}$.
% If we take $z_j^+=0$ or $z_j^-=0$ for all $j$, then
% $(z_j^++z_j^-)=\sum_i|\langle v_i,x^{(j)} \otimes y^{(j)}\rangle|=|\langle v,x^{(j)} \otimes y^{(j)}\rangle|$.
Then it follows that there exists $v$ such that
\begin{equation}\label{eqn:contradict_using_anticonc}
\langle v,P\rangle + \underbrace{D\sum_{j \in [4k]}|\langle v,x^{(j)} \otimes y^{(j)}\rangle|}_{(i)}<0 \;.
\end{equation}
To contradict Equation~\eqref{eqn:contradict_using_anticonc}, it suffices to show that with high probability
term (i) is at least $\frac{c_1}{\sqrt{\eta}\alpha}\Norm{v}_F \geq \Iprod{P,v}$,
where the inequality follows from Lemma \ref{lem:existence_2_tensor}.
Let $Q$ be an orthonormal basis for the span of $\Sigmaa'_i$ for all $i \in[k]$, and thus $QQ^\top$
is the corresponding projection matrix.
W.l.o.g., we can assume $\Norm{v}_F = 1$
and, since $ Q Q^\top $ is a projection,
we have that $\Norm{Q Q^\top v}_F\leq 1$. Let $\tilde{v} = QQ^\top v$.

Alternatively, it suffices to show that
\begin{equation}
\label{eqn:to_obtain_contradiction}
\sum_{j \in [4k]}\Iprod{ \tilde{v} ,  x^{(j)} \otimes y^{(j)}   }  \leq \Paren{\frac{c_1 }{\sqrt{\eta} \alpha D }}
\end{equation}
holds with small probability.
We can construct $\calC$, a $\gamma$-cover for all such $\tilde{v}$,
where $\gamma = \Paren{\frac{c'_1 }{ t k^2 \sqrt{\eta} \alpha D}}$.
Since this subspace (of $\mathbb{R}^{d^2}$) is $k$-dimensional, we have that
$\abs{\calC} = \bigO{ 1/ \gamma }^{k}$. Replacing $\tilde{v}$ by the closest point in $\calC$,
denoted by $\tilde{v}'$, it suffices to show
\begin{equation}
\sum_{j \in [4k]}\Iprod{ \tilde{v}' ,  x^{(j)} \otimes y^{(j)}   }  = \sum_{j \in [4k]}\Iprod{ \tilde{v} ,  x^{(j)} \otimes y^{(j)}   } + \sum_{j \in [4k]}\Iprod{ \tilde{v}  - \tilde{v}',  x^{(j)} \otimes y^{(j)}   }   \leq \Paren{\frac{2c_1 }{\sqrt{\eta} \alpha D}}
\end{equation}
holds with small probability.
Each term in $\sum_{j \in [4k]}\Iprod{ \tilde{v}' ,  x^{(j)} \otimes y^{(j)}}$ is a random bi-linear form
given by $z_j = \sum_{\ell, p\in [d]} \tilde{v}'_{\ell,p} x^{(j)}_{\ell}y^{(j)}_{p}$.
Then, we have that $\expecf{}{z_j} = 0$ and
\begin{equation*}
\begin{split}
\expecf{}{z^2_j} = \expecf{}{ \Paren{\sum_{\ell, p\in [d]} \tilde{v}'_{\ell,p} x^{(j)}_{\ell}y^{(j)}_{p}}^2} & = \sum_{\ell, \ell', p, p'} \expecf{}{\tilde{v}'_{\ell,p} \tilde{v}'_{\ell',p'} x^{(j)}_{\ell} x^{(j)}_{\ell'} y^{(j)}_{p} y^{(j)}_{p'} } \\
& = \sum_{\ell, p\in [d] } \Paren{\tilde{v}'_{\ell,p}}^2 \cdot \expecf{}{ \Paren{x^{(j)}_{\ell}}^2} \cdot  \expecf{}{ \Paren{y^{(j)}_{p}}^2}\\
& = 1 \;,
\end{split}
\end{equation*}
where the last equality follows from $\Norm{\tilde{v}'}_F = 1$.
% w Using Carbery-Wright, we have
% \begin{equation*}
% \Pr\left[ z_j \leq \zeta \expecf{}{z_j^2} \right] \leq c_5 \sqrt{\zeta}
% \end{equation*}
% \anote{need citation for the above inequality, or prove it.}
Using Lemma \ref{lem:anti-concentration_of_bilinear_forms} with $\zeta = \frac{2c_1 }{\sqrt{\eta} \alpha D}$,
\begin{equation}
\Pr\left[ \abs{z_j} \leq \frac{2c_1 }{\sqrt{\eta} \alpha D}\right] \leq c_5 \Paren{\frac{2c_1 }{\sqrt{\eta} \alpha D}}^{1/2} \;.
\end{equation}
Since the $z_j$'s are independent, we can repeat $t$ times, and conclude that
\begin{equation}
\Pr\left[ \sum_{j \in [4k]}\Iprod{ \tilde{v}' ,  x^{(j)} \otimes y^{(j)}   }
\leq \frac{2c_1 }{\sqrt{\eta} \alpha D}\right] \leq \Paren{\frac{2c_1 }{\sqrt{\eta} \alpha D}}^{t/2} \;.
\end{equation}
Since the above argument holds for any $u \in \calC$, we can union bound over all elements in the cover $\calC$,
and the probability that there exists a $\tilde{v}'$ in the cover that does not satisfy Equation~\eqref{eqn:to_obtain_contradiction}
is $\Paren{  t k^2 \sqrt{\eta} \alpha D }^{k} \cdot \Paren{\frac{2c_1 }{\sqrt{\eta} \alpha D}}^{t/2}$.
Setting $D = \bigO{k^4/ (\sqrt{\eta} \alpha)}$ suffices to
conclude that with probability at least $1-1/{\poly(k)}$, the primal is feasible.
\end{proof}

% We note that the equations defining $b_j$ define a linear program that will have a solution unless the dual does. The dual linear program in this case asks for a $2$-tensor $v$ so that
% $$
% \sum_{i=1}^{2j} |v\cdot (x^j\otimes y^j)| \leq  (1/D)(v\cdot P) \leq (1/2kM)^3 |v|_2,
% $$
% for $M$ a sufficiently large constant. We note that we can assume here that $v$ is a unit norm element of the span of the $\Sigmaa_i'$. Let $\mathcal{C}$ be a $(1/2kM)^3$-cover of this set of size $O(kM)^{3k}$. We note that if the above has a solution, replacing $v$ by $v'$, it's closest representative in $\mathcal{C}$, we have that
% $$
% \sum_{i=1}^{2j} |v'\cdot (x^j\otimes y^j)| \leq (1/2kM)^2.
% $$
% We claim that for each $v'\in\mathcal{C}$ that this happens with probability substantially smaller than $O(kM)^{-3k}$. In particular, for it to occur, it must be the case that $|v'\cdot (x^j\otimes y^j)| \leq (1/2kM)^2$ for all $j$. However, for a given $j$, $v'\cdot (x^j\otimes y^j)$ is a bilinear polynomial in $x^j$ and $y^j$ with mean square equal to $1$. From this it is easy to show that this happens with probability $O(1/kM)^2$. Thus, the probability that it holds for all $j$ is $O(1/kM)^{4k}$.




\begin{proof}[Proof of Proposition~\ref{prop:tensor_decomposition_upto_lowrank}]
We begin by bounding the Frobenius norm of $\hat{T}_4$.
Let $T_4 = \E[h_4(\calX)]$. It  then follows from Lemma \ref{HermiteExpectationLem} that
\begin{equation}
\label{eqn:expected_4th_hermite_tensor}
T_4 = \sym\left(\sum_{i=1}^k w_i \left(3\Sigmaa_i\otimes \Sigmaa_i +6\Sigmaa_i\otimes \mu_i^{\otimes 2}+\mu_i^{\otimes 4} \right) \right) \;.
\end{equation}
Further, $\Norm{\Sigmaa_i\otimes \Sigmaa_i}_F \leq \Norm{\Sigmaa_i}^2_F\le\Delta^2$,
$\Norm{\Sigmaa_i\otimes \mu_i^{\otimes 2}}_F \leq \Norm{\Sigmaa_i}_F\Norm{\mu_i}^2_2\le4\Delta/\alpha$,
and $\Norm{\mu_i^{\otimes 4}}_F \leq \Norm{\mu_i}^4_2\le16/\alpha^2$.
Since $T_4$ is an average of terms of the form $\Sigmaa_i^{\otimes 2}, \Sigmaa_i\otimes \mu_i^{\otimes 2}$
and $\mu_i^{\otimes 4}$, and each such term is upper bounded, we can conclude that
$\Norm{T_4}_F = \bigO{\Delta^2 + 1/\alpha^2 }$, and by the triangle inequality that
$\Norm{ \hat{T}_4 }_F \leq \bigO{\Delta^2 + 1/\alpha^2 + \eta}$.
%Note that $|T|_F  \leq M = O(\Delta^2+1/\alpha^2+1)$.
%This is because $\E[h_4(X)]$ is an average of terms of the form $\Sigmaa_i^{\otimes 2}, \Sigmaa_i\otimes \mu_i^{\otimes 2}$ and $\mu_i^{\otimes 4}$. Since each of these have an appropriate bound, this bounds $|\E[h_4(X)]|_2$ and thus $T$.
% Let
% $$
% T_4 := \E[h_4(X)] = \sym\left(\sum_{i=1}^k w_i \left(3\Sigmaa_i\otimes \Sigmaa_i +6\Sigmaa_i\otimes \mu_i^{\otimes 2}+\mu_i^{\otimes 4} \right) \right).
% $$
Let $\Sigmaa_i'=\Sigmaa_i+\mu_i^{\otimes 2}$ and let $T_4':= \sum_{i=1}^k w_i \left(\Sigmaa_i'\otimes \Sigmaa_i' \right)$.
We can then rewrite Equation~\eqref{eqn:expected_4th_hermite_tensor} as follows:
\begin{equation}
\label{eqn:rewrite_4th_hermite_tensor}
T_4 = \sym\left(\sum_{i=1}^k w_i \left(3\Sigmaa_i'\otimes \Sigmaa_i' -2\mu_i^{\otimes 4} \right) \right) \;.
\end{equation}
% $$
% T_4 = \sym\left(\sum_{i=1}^k w_i \left(3\Sigmaa_i'\otimes \Sigmaa_i' -2\mu_i^{\otimes 4} \right) \right).
% % $$
% Finally,
% $$
% T_4':= \sum_{i=1}^k w_i \left(\Sigmaa_i'\otimes \Sigmaa_i' \right).
% $$
For $j \in [4k]$, let $x^{(j)}, y^{(j)} \sim \calN(0, I)$. Collapsing two modes of $\hat{T}_4$, it follows from Equation \eqref{eqn:rewrite_4th_hermite_tensor} that for any fixed $j$,
\begin{equation}
\label{eqn:symmeterizing_hermite_tensor}
\begin{split}
\hat{T}_4\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}} &= \Paren{\hat{T}_4 - T_4}\hspace{-0.06in}\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}} + T_4\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}}\\
&  = \Paren{\hat{T}_4 - T_4}\hspace{-0.06in}\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}}  + \sym\left(\sum_{i=1}^k w_i \left(3\Sigmaa_i'\otimes \Sigmaa_i' -2\mu_i^{\otimes 4} \right) \right)\Paren{\cdot, \cdot, x^{(j)}, y^{(j)}} \\
& =  \Paren{\hat{T}_4 - T_4 + T'_4}\hspace{-0.06in}\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}} + \sum_{i\in [k]} w_i \Paren{\Sigmaa_i' x^{(j)}} \otimes \Paren{\Sigmaa_i' y^{(j)}} \\
& \hspace{0.2in} + \sum_{i\in [k]} w_i\Paren{\Sigmaa_i' y^{(j)}} \otimes \Paren{\Sigmaa_i' x^{(j)}}  + \sum_{i \in [k]} w_i \Paren{ -2 \mu_i^{\otimes 2} \Iprod{\mu_i, x^{(j)}} \Iprod{\mu_i, y^{(j)}} } \;,
\end{split}
\end{equation}
where we use that $\sym(\cdot)$ is a linear operator satisfying $\sym\Paren{\mu_i^{\otimes 4}} = \mu_i^{\otimes 4}$, and
\begin{equation*}
\sym\Paren{ \Sigmaa'_i \otimes \Sigmaa'_i } = \frac{1}{3} \Sigmaa'_i  \otimes \Sigmaa'_i + \frac{1}{3} \Sigmaa'_i  \oplus \Sigmaa'_i + \frac{1}{3} \Sigmaa'_i  \ominus \Sigmaa'_i
\end{equation*}
where for indices $(i_1, i_2, i_3, i_4)$, $\Paren{\Sigmaa'_i  \oplus \Sigmaa'_i}\Paren{i_1, i_2, i_3, i_4} = \Paren{\Sigmaa'_i  \otimes \Sigmaa'_i}\Paren{i_1, i_3, i_2, i_4}$ and $\Paren{\Sigmaa'_i  \ominus \Sigmaa'_i}\Paren{i_1, i_2, i_3, i_4} = \Paren{\Sigmaa'_i  \otimes \Sigmaa'_i}\Paren{i_1, i_4, i_2, i_3}$.
%We now use Lemma \ref{lem:concentration_of_low_degree_gaussians} \anote{add stand alone lemma on bounding random bi-linear form of $\hat{T}_4 - T_4$.} to conclude that with probability at least $1-1/\poly(k)$,
%Rearranging Equation \eqref{eqn:symmeterizing_hermite_tensor}, we have
%\begin{equation}
%\label{eqn:split_frob_low_rank}
%\begin{split}
%\Paren{\hat{T}_4 - T'_4}\hspace{-0.06in}\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}}
%& =  \Paren{\hat{T}_4 - T_4}\hspace{-0.06in}\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}} + \sum_{i\in [k]} w_i \Paren{\Sigmaa_i' x^{(j)}} \otimes \Paren{\Sigmaa_i' y^{(j)}} \\
%& \hspace{0.2in} + \sum_{i\in [k]} w_i\Paren{\Sigmaa_i' y^{(j)}} \otimes \Paren{\Sigmaa_i' x^{(j)}}  + \sum_{i \in [k]} w_i \Paren{ -2 \mu_i^{\otimes 2} \Iprod{\mu_i, x^{(j)}} \Iprod{\mu_i, y^{(j)}} } \;.
%\end{split}
%\end{equation}
%such that  $\Norm{\Paren{\hat{T}_4 - T_4}\hspace{-0.06in}\Paren{ \cdot, \cdot , x^{(j)},  y^{(j)}} }_F \leq \tilde{\mathcal{O}}\Paren{\eta}$ and the remaining terms have rank $\bigO{k}$.


% Next, we note that for random Gaussians $x$ and $y$ that with probability $1-1/(10k)$:
% \begin{align*}
% T_{i_1i_2i_3i_4}x_{i_3}y_{i_4} &= (T-T_4)_{i_1i_2i_3i_4}x_{i_3}y_{i_4}+(T_4)_{i_1i_2i_3i_4}x_{i_3}y_{i_4}\\
% &= O(\eta\log(k))+(T_4')_{i_1i_2i_3i_4}x_{i_3}y_{i_4}+3\sum_{i=1}^k w_i[ (\Sigmaa_i' x)\otimes (\Sigmaa_i' y)+ (\Sigmaa_i' y)\otimes (\Sigmaa_i' x)]\\ & \ \ \ \  \ \ \ +\sum_{i=1}^k w_i\left(-2\mu_i^{\otimes 2} (\mu_i\cdot x)(\mu_i\cdot y) \right).
% \end{align*}
% This is a matrix of Frobenius norm $ O(\eta\log(k))$ plus a rank $O(k)$ matrix plus $(T_4')_{i_1i_2i_3i_4}x_{i_3}y_{i_4}.$

% We now show that for each $i \in [k]$, with probability at least $1-1/\poly(k)$, over the choice of $x^{(j)}$ and $y^{(j)}$, there exist a sequence of $t$ reals, $b_j \in [-D, D]$, such that $\sum_{j \in [t]} b_j T'_4\Paren{ \cdot, \cdot, x^{(j)}y^{(j)} } = \Sigmaa_i + P_i $, where $P_i$ has small Frobenius norm.

Next, it follows from Lemma \ref{lem:existence_2_tensor} that there exists a matrix $\tilde{P}_i$ such that
$\Norm{\tilde{P}_i}_F = \bigO{1/(\sqrt{\eta} \alpha)}$ and
$\Norm{T'_4\Paren{\cdot, \cdot, \tilde{P}_i} - \Sigmaa'_i }_F = \bigO{\sqrt{\eta/\alpha}}$.
Then, we use Lemma \ref{lem:existence_of_bilinear} to conclude that $\tilde{P}_i$ lies in the vector space
given by $\cup_{i \in [k]} \textrm{span}\Paren{ \Sigmaa'_i }$.
Formally, with probability at least $1-1/\poly(k)$, there exists a sequence of $b_j \in [-D,D]$,
for $j \in [4k]$, such that $T'_4\Paren{\cdot,\cdot, \sum_{j \in[4k] } b_j x^{(j)} \otimes y^{(j)} } = T'_4\Paren{\cdot, \cdot, \tilde{P}_i}$.
We now cover the interval $[-D, D]$ using a set $\calC$, with points spaced at intervals of length
$\gamma = \bigO{ \frac{\sqrt{\eta}}{\alpha k\Paren{\Delta^4 + 1/\alpha^4}} }$.
For each $b_j$, we pick the closest $a_j \in \calC$, and  thus,
\begin{equation}
\label{eqn:closeness_T'_and_S'}
\begin{split}
\Norm{ T'_4\Paren{\cdot,\cdot, \sum_{j \in[4k] } a_j x^{(j)} y^{(j)} }  - \Sigmaa'_i}_F & \leq  \Norm{ T'_4\Paren{\cdot,\cdot, \sum_{j \in[4k] } b_j x^{(j)}\otimes y^{(j)} }  - \Sigmaa'_i}_F + \Norm{ T'_4\Paren{\cdot,\cdot, \sum_{j \in[4k] } (b_j-a_j)x^{(j)}\otimes y^{(j)} } }_F\\
& \leq \bigO{\sqrt{\eta/\alpha} } +\bigO{\gamma\Delta^2}
\le \bigO{\sqrt{\eta/\alpha} } \;.
\end{split}
\end{equation}
Further, the probability of picking each $a_j$ correctly by uniformly sampling is $\Paren{\gamma/D}^t$.
Taking the linear combinations with coefficients $a_j$ in Equation \eqref{eqn:symmeterizing_hermite_tensor}, we have
\begin{equation} \label{eqn:final_guarantee_split_frob_low_rank}
\begin{split}
\hat{T}_4\Paren{ \cdot, \cdot , \sum_{j\in [4k]} a_j x^{(j)}\otimes  y^{(j)}} - \Sigmaa_i
& =  \Paren{\hat{T}_4 - T_4 + T'_4 }\hspace{-0.04in}\Paren{ \cdot, \cdot , \sum_{j \in [4k]}a_j x^{(j)} \otimes y^{(j)}} - \Sigmaa'_i - \mu_i \otimes \mu_i  \\
& \hspace{0.2in} + \sum_{j \in [4k]} a_j \sum_{i\in [k]} w_i \Paren{\Sigmaa_i' x^{(j)}} \otimes \Paren{\Sigmaa_i' y^{(j)}} + \sum_{j \in [4k]} a_j \sum_{i\in [k]} w_i\Paren{\Sigmaa_i' y^{(j)}} \otimes \Paren{\Sigmaa_i' x^{(j)}}  \\
& \hspace{0.2in}  +\sum_{j \in [4k]} a_j \sum_{i \in [k]} w_i \Paren{ -2 \mu_i^{\otimes 2} \Iprod{\mu_i, x^{(j)}} \Iprod{\mu_i, y^{(j)}} } \;.
\end{split}
\end{equation}
Setting $P_i = \Paren{\hat{T}_4-T_4 + T'_4}\Paren{\cdot,\cdot, \sum_{j \in[4k] } a_j x^{(j)} y^{(j)}} - \Sigmaa'_i$, it follows from Lemma \ref{lem:concentration_of_low_degree_gaussians} that with probability at least $1-1/d$, $\Paren{\hat{T}_4 -T_4}\Paren{\cdot,\cdot, \sum_{j \in[4k] } a_j x^{(j)} y^{(j)}}$ has Frobenius norm $\bigO{k D \eta}$ and it follows from Equation \eqref{eqn:closeness_T'_and_S'} that with probability at least $1-1/d$, $T'_4\Paren{\cdot,\cdot, \sum_{j \in[4k] } a_j x^{(j)} y^{(j)}} - \Sigmaa'_i$ has Frobenius norm $\bigO{\sqrt{\eta/\alpha}}$. Setting the remaining terms to $Q_i$, with probability at least $1- \Omega(1/d)$ we can bound their Frobenius norm as follows:
\begin{equation}
\begin{split}
\Norm{Q_i}_F & \leq \Norm{\mu_i \otimes \mu_i}_F + \Norm{ \Paren{\sum_{i \in [k]} w_i \Sigmaa'_i \oplus \Sigmaa'_i + w_i\Sigmaa'_i\ominus \Sigmaa'_i -2 w_i\mu_i^{\otimes 4} }\Paren{\cdot, \cdot, \sum_{j \in [4k]} a_j x^{(j)} y^{(j)} }  }_F \\
& \leq \frac{4}{\alpha} + \Paren{2 \max_{i\in k} \Norm{\Sigmaa'_i}^2_F + 32/\alpha^2 }\cdot \Norm{\tilde{P}}_F \\
& \leq \frac{4}{\alpha}+ \bigO{ \frac{1}{\sqrt{\eta}\alpha} \Paren{\Delta +\frac{1}{\alpha}}^2}\\
& \le \bigO{\frac{1+\Delta^2}{\sqrt{\eta}\alpha^3}} \;,
\end{split}
\end{equation}
where the first inequality follows from the triangle inequality,
the second follows from our assumptions that $\Norm{\mu_i}_2 \leq 2/\sqrt{\alpha}$ and
$\sum_{j \in [4k]} a_j x^{(j)} y^{(j)} = \tilde{P}_i$ in the span of the $\Sigmaa'_i$,
and the third inequality follows from the definition of $\Sigmaa'_i$,
the bound on $\Norm{\tilde{P}}_F$ and the bound on $\Norm{\Sigmaa_i -I}_F$.
\end{proof} 

==> weight-gap.tex <==
\begin{lemma}
Suppose $0<w_1\le \cdots\le w_k<1$ are $k$ real numbers such that $\sum_i w_i=1$. Define $f_{k-\ell}=1/(10^\ell C^{k!/(k-i)!}\mathrm{sf}(k)/\mathrm{sf}(k-i))$. If $\epsilon\le1/k^{1/c^{k+1}}$ for some $c<1$, then one of the following is true:
\begin{enumerate}
\item $w_i\ge\epsilon^c$ for all $i$
\item there exists $i\le k-1$ such that $w_i< \epsilon^{c^i}$ and $w_{i+1}\ge\epsilon^{c^{i+1}}$.
\end{enumerate}
\end{lemma}

\begin{proof}
We may assume $w_1<\epsilon^c$. Then we will prove 2 by contradiction. $w_1<\epsilon^c$ implies that $w_2<\epsilon^{c^2}$. Inductively, we have
$w_k <\epsilon^{c^k}$. Given that $\sum_i w_i=1$, we also have $w_k\ge 1/k$. Combining these two inequalities gives $\epsilon^{c^k}>1/k$,
which contradicts to the assumption that $\epsilon\le1/k^{1/c^k}$.
\end{proof}
